Toward a Better Understanding of Probabilistic Delta Debugging

Given a list L of elements and a property that L exhibits, ddmin is a well-known test input minimization algorithm designed to automatically eliminate irrelevant elements from L. This algorithm is extensively adopted in test input minimization and software debloating. Recently, ProbDD, an advanced variant of ddmin, has been proposed and achieved state-of-the-art performance. Employing Bayesian optimization, ProbDD predicts the likelihood of each element in L being essential, and statistically decides which elements and how many should be removed each time. Despite its impressive results, the theoretical probabilistic model of ProbDD is complex, and the specific factors driving its superior performance have not been investigated. In this paper, we conduct the first in-depth theoretical analysis of ProbDD, clarifying trends in probability and subset size changes while simplifying the probability model. Complementing this analysis, we perform empirical experiments, including success rate analysis, ablation studies, and analysis on trade-offs and limitations, to better understand and demystify this state-of-the-art algorithm. Our success rate analysis shows how ProbDD addresses bottlenecks of ddmin by skipping inefficient queries that attempt to delete complements of subsets and previously tried subsets. The ablation study reveals that randomness in ProbDD has no significant impact on efficiency. Based on these findings, we propose CDD, a simplified version of ProbDD, reducing complexity in both theory and implementation. Besides, the performance of CDD validates our key findings. Comprehensive evaluations across 76 benchmarks in test input minimization and software debloating show that CDD can achieve the same performance as ProbDD despite its simplification. These insights provide valuable guidance for future research and applications of test input minimization algorithms.

==> acm_template/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> acm_template/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> alg/counterdd_size.tex <==

\begin{algorithm}[h]
    \small
\DontPrintSemicolon
\SetKwInput{KwData}{Input}
\SetKwInput{KwResult}{Output}
\caption{\protect\AlgComputeSize{$\textit{counter}, \myprobability{0}{}$
}}
\label{alg:counterdd_size}

\KwData{$\textit{counter}$ : the counter recording the number a element has been attempted for deletion.}
\KwData{\pinit: the initial prior probability provided by the user.}
\KwResult{the subset size \mysize{}{} with maximum reduction expectation.}
\tcc{Based on  \cref{equation:counter}, subset size \mysize{}{} with maximum reduction expectation can be computed by the
%\cn{frequency?}\mz{done, replaced all frequency with times}
times the elements has been tried for deletion, if the initial probability is given.}
\If{$counter == 0$}{
	\tcc{Since $-1 / \ln(1 - \myprobability{0}{})$ is decimal, we need to evaluate two nearest integers to it.}
	$\mysize{f}{} \gets \lfloor -1 / \ln(1 - \myprobability{0}{}) \rfloor$ \;
	$\mysize{c}{} \gets \lceil -1 / \ln(1 - \myprobability{0}{}) \rceil$ \;
	$gain_{f} \gets \mysize{f}{} \times (1 - \myprobability{0}{})^{\mysize{f}{}}$ \;
	$gain_{c} \gets \mysize{c}{} \times (1 - \myprobability{0}{})^{\mysize{c}{}}$ \;
	\If{$gain_{f} > gain_{c}$}{
		\Return \mysize{f}{} \;
	}
	\Else{
		\Return \mysize{c}{} \;
	}
}
\Else{
	\Return $\lfloor (1 - e^{-1}) \times \AlgComputeSize(counter - 1) \rfloor$ \;
}
\end{algorithm}


==> alg/ddmin.tex <==

\begin{algorithm}[h]
    \small
	\DontPrintSemicolon
	\SetKwInput{KwData}{Input}
	\SetKwInput{KwResult}{Output}
	\caption{\protect\AlgDdmin{$L, \psi$}}
	\label{alg:ddmin}

	\KwData{$L$: a list of element to be reduced.}
	\KwData{$\psi: \searchspace \rightarrow \boolspace$:
		the property to be preserved by $L$.
	}
	\KwResult{the minimized list that still exhibits the property $ \psi $ .}

$\lmin \gets L$\;
$n \gets 2$ \tcc{Initialize n as the number of subsets}
\While{True}{
	$\textit{reduced} \gets \textit{false}$ \;
	\tcc{Partition $\lmin$ into n subsets as evenly as possible and store them in a list S}
	$S \gets $ \textit{n subsets from \lmin} \;

	\tcc{Step1: Reduce-to-subset. Check if any single subset can pass the property check}
	\ForEach{$\textit{subset}$ \textbf{in} $\textit{S}$}{
		\label{alg:ddmin:step1_start}
		\If{$\psi(\textit{subset})$ is true}{
			$\lmin \gets \textit{subset}$\;
			$n \gets 2$\;
			$\textit{reduced} \gets \textit{true}$ \;
			\Break \;
		}
	}
	\If {$\textit{reduced}$ is true} {
		\Continue \;
	}
	\label{alg:ddmin:step1_end}

	\tcc{Step2: Reduce-to-complement. Check if any complement of a subset can pass the property check}
	\ForEach{$\textit{subset}$ \textbf{in} $\textit{S}$}{
		\label{alg:ddmin:step2_start}
		$\textit{complement} \gets \lmin \setminus \textit{subset} $ \;
		\If{$\psi(\textit{complement})$ is true}{
			$\lmin \gets \textit{complement}$\;
			$n \gets n - 1$\;
			$\textit{reduced} \gets \textit{true}$ \;
			\Break \;
		}
	}
	\If {$\textit{reduced}$ is true} {
		\Continue \;
	}
	\label{alg:ddmin:step2_end}

	\tcc{Step3: Subdivide. Divide subsets into finer granularity if possible}
	\If{$n = |\lmin|$} {
		\label{alg:ddmin:step3_start}
		\Break \;
	}
	\Else {
		$n \gets  \textit{Min}(2 \times n, |\lmin|)$ \;
	}
	\label{alg:ddmin:step3_end}
}

\Return $\lmin$\;

\end{algorithm}


==> alg/ddmin_opts.tex <==

\begin{algorithm}[h]
    \small
	\DontPrintSemicolon
	\SetKwInput{KwData}{Input}
	\SetKwInput{KwResult}{Output}
	\caption{\protect\AlgDdminWithOpts{$L, \psi, T$}}
	\label{alg:ddmin_opts}

	\KwData{$L$: a list of element to be reduced.}
	\KwData{$\psi: \searchspace \rightarrow \boolspace$:
		the property to be preserved by $L$.
	}
	\KwData{$T$: the threshold of \myopt.}
	\KwResult{the minimized list that still exhibits the property $ \psi $ .}

$\lmin \gets L$\;
$n \gets 2$\;

\While{True}{
	$\textit{reduced} \gets \textit{false}$ \;
	$\textit{subset list} \gets $ \textit{n subsets from \lmin} \;

	\begin{mdframed}[
		backgroundcolor=green!20,
		linewidth=0pt,
		innerleftmargin=0pt,
		innertopmargin=0pt,
		innerrightmargin=0pt,
		innerbottommargin=0pt,
		skipabove=-3mm,
		skipbelow=-3mm,
		leftmargin=0cm, % Adjust left margin
		rightmargin=1cm  % Adjust right margin
		]
		\tcc{\myopt enables the following code}
		\If{$\exists \textit{subset} \in \textit{subset list}, |\textit{subset}| > T$} {
			$n \gets  \textit{Min}(2 * n, |\lmin|)$ \;
			\Continue \;
		}
	\end{mdframed}
%	\vspace{-1.5mm}
	\begin{mdframed}[
	backgroundcolor=gray!20,
	linewidth=0pt,
	innerleftmargin=0pt,
	innertopmargin=0pt,
	innerrightmargin=0pt,
	innerbottommargin=0pt,
	skipabove=-3mm,
	skipbelow=-3mm,
	leftmargin=0cm, % Adjust left margin
	rightmargin=1cm  % Adjust right margin
	]
	\tcc{\complementonly skips the following code}
	\tcc{Step1: Reduce-to-subset}
	\ForEach{$\textit{subset}$ \textbf{in} $\textit{subset list}$}{
		\If{$\psi(\textit{subset})$ is true}{
			$\lmin \gets \textit{subset}$\;
			$n \gets 2$\;
			$\textit{reduced} \gets \textit{true}$ \;
			\Break \;
		}
	}
	\If {$\textit{reduced}$ is true} {
		\Continue \;
	}
	\end{mdframed}
%	\vspace{-3mm}
	\tcc{Step2: Reduce-to-complement}
	\ForEach{$\textit{subset}$ \textbf{in} $\textit{subset list}$}{
		\begin{mdframed}[
		backgroundcolor=blue!20,
		linewidth=0pt,
		innerleftmargin=0pt,
		innertopmargin=0pt,
		innerrightmargin=0pt,
		innerbottommargin=0pt,
		skipabove=-3mm,
		skipbelow=-3mm,
		leftmargin=0cm, % Adjust left margin
		rightmargin=2cm  % Adjust right margin
		]
		\tcc{\onepass enables the following code}
		\If{$\textit{subset has been tried}$} {
			\Continue \;
		}
	\end{mdframed}
%	\vspace{-3mm}
		$\textit{complement} \gets \lmin \setminus \textit{subset} $ \;
		\If{$\psi(\textit{complement})$ is true}{
			$\lmin \gets \textit{complement}$\;
			$n \gets n - 1$\;
			$\textit{reduced} \gets \textit{true}$ \;
			\Break \;
		}
	}
	\If {$\textit{reduced}$ is true} {
		\Continue \;
	}

	\tcc{Step3: Subdivide. Divide subsets into finer granularity if possible}
	\If{$n = |\lmin|$} {
		\Break \;
	}
	\Else {
		$n \gets  \textit{Min}(2 \times n, |\lmin|)$ \;
	}
}

\Return $\lmin$\;
\end{algorithm}


==> data_availability.tex <==
For experiment replication, we release the source code and the
replication process at \codeurl.

==> discussion.tex <==
In this section, we discuss about global optimal result, and threats to validity.

\subsection{The Existence of the Optimal Result}
For test input minimization tasks, a global minimal result exists but is expensive to obtain, as it is an NP-complete problem~\cite{misherghi2006hdd}. To simplify the problem, \probdd follows the assumption of unambiguity. In other words, the intersection of any two variants satisfying the property still satisfy the property, and the global minimum is the common minimum subset of all variants that meet the conditions. Although this assumption serves as one of the theoretical foundations of \probdd, we find it not very practical, because in various test input minimization scenarios, local minimal results are generally prevalent.


%\subsection{Discrepancies from the Original \probdd Study}
%Our work began with the study of the \probdd paper, starting with investigating why the performance of \probdd is good, and gradually deriving the simplified model and \myopt. However, our results from \compilerbench and \chiselbench only conclude that \probdd is faster than \ddmin, while cannot prove that \probdd can achieve a smaller size, which is
%claimed in \probdd paper.
%Such a discrepancy could be attributed to a variety of factors, such as differences in experimental setup or data processing. Specifically, the previous work only kept cases within a runtime of 3 hours, while our evaluation provides results for all runtime, making our findings more reliable.

%\subsection{Future Work}
%Our work has demonstrated the practicality of \myopt, but determining a threshold $T$ to decide from what size \ddmin should start remains an empirical question. Therefore, for future work, we plan to investigate whether statistics and probabilities can be used to record the success rate of each size, and then derive the threshold with the highest expected success rate.
%Additionally, all evaluations were conducted at the list level, \ie, applied to each layer of the \hdd, and ignored the information that the tree structure itself could provide. In the future, we plan to consider the sub-tree size corresponding to each element in order to obtain even smaller programs.


\subsection{Threats to Validity}
\myparagraph{External Validity}
One threat to external validity is that the evaluation might not be representative. To mitigate this threat, we selected the benchmarks used by \probdd, namely \benchmarknum
benchmark programs from compiler bugs and software debloating, which respectively represent reduction on randomly generated programs that trigger compiler bugs and command-line tool source code written by humans. Moreover, all reduced code is written in C/C++, so it cannot be claimed that our results are representative of other programming languages. Nevertheless, we believe that given the popularity of C/C++, it has a certain degree of representativeness. Even if we only focus on reducing C programs, we believe our work still makes a significant contribution.

\myparagraph{Internal Validity}
The main internal threat comes from the simplifying assumptions we made for \probdd. We assumed no element would be removed and that the input list could always be evenly divided into subsets. Though ideal, this assumption facilitate mathematical derivation. We believe their impact on the results is minimal.
Besides, removing elements only affects size, not the probabilities of other elements in \probdd's algorithm.
Another assumption is that the list length is always divisible by the subset size. In reality, if this assumption does not hold,
the remaining elements will be combined with the next round's initial elements to form a new subset.
This may cause a slight difference in probability or counter updates, but it is unlikely to significantly impact the results.
Our experiments support the validity of our theory and simplification,
as \myalgorithm's performance is not significantly different from \probdd in terms of program size and execution time.


==> evaluation/evaluation/rq5.tex <==
todo

==> evaluation/rq1.tex <==
\input{table/rq1_all}
\input{table/rq1_p_value}

\finding{For efficiency, \probdd and \proj are
	significantly superior to
	\ddmin. For effectiveness, \probdd and \proj exhibit similar performance
	to
	\ddmin. Despite being much simplified in algorithm design, \proj always
	achieves
	comparable performance to \probdd,
	indicating the non-necessity of probability.
}

% settings
To answer this research question, we evaluate \ddmin, \probdd, and \proj
with the four benchmark suites, containing \benchmarkNumTotal
benchmarks in total.
Following the settings of \probdd~\cite{wang2021probabilistic},
we set the empirically estimated remaining rate as the initialization
probability
\pinit, specifically, 0.1 for \cBenchmarkNameShort and
\debloatBenchmarkNameShort, 2.5e-3 for \xmlBenchmarkNameShort, and 1e-7
for \stringBenchmarkNameShort.
Same as \probdd's paper, we employ three hours (10,800
seconds) as the timeout
threshold.
%\victor{why shall we choose 3 hours as the limit? any reference?
%I am wondering whether this will affect the results and conclusions.
% } \mz{we follow the original probdd paper. I added it}
% \victor{if we increase the size, I think we will have more finished ones.
% Will this bring benefits to \proj?} \mz{No. I have thought about every tricks
% that can benefit cdd, we should give up attempts to prove cdd is better
% than probdd, as they are equivalent. I can use cdd to prove that probability
% is useless, and further reveal which part is actually useful }
If the algorithm does not complete a benchmark within the time
limit,
the
smallest result achieved and the corresponding query number are still
recorded. Due to the significant differences between
completed and uncompleted results, we only consider benchmarks
completed by all algorithms when calculating averages.
The detailed results are shown in
\cref{table:rq1_firsthalf} and \cref{table:rq1_secondhalf}, and the overall comparisons among algorithms are
displayed in \cref{table:rq1_p_value}.

% time and test
\myparagraph{Efficiency}
As shown in  \cref{table:rq1_p_value}, \probdd and \proj are significantly
more efficient than \ddmin.
\proj completes the most benchmarks, totaling
\benchmarkNoTimeoutNumProj, followed by \probdd
with \benchmarkNoTimeoutNumProbdd benchmarks completed,
and \ddmin with
\benchmarkNoTimeoutNumDdmin benchmarks completed.
On benchmarks that can be completed by all algorithms, \probdd and \proj
require
\benchmarkNoTimeoutTimeDecRateProbddVsDdmin and
\benchmarkNoTimeoutTimeDecRateCddVsDdmin less time,
\benchmarkNoTimeoutQueryDecRateProbddVsDdmin and
\benchmarkNoTimeoutQueryDecRateCddVsDdmin fewer queries,
respectively.
%Even on those benchmarks where all algorithms timeout,
%\probdd and \proj still perform
%\benchmarkTimeoutQueryDecRateProbddVsDdmin
%and \benchmarkTimeoutQueryDecRateCddVsDdmin fewer tests than
%\ddmin.
%\zy{So it means \probdd and \proj issue fewer tests than \ddmin in the
%same period of time?
%How to interpret this result?}
%\cn{I have the same question.}
Meanwhile, \proj performs on par with \probdd \wrt execution time and
query number,
with a p-value greater than 0.05, indicating insignificance between these
two
algorithms. \proj is expected to perform on par with \probdd since it is
designed to provide further insight and unravel the complexities of
\probdd, rather than to surpass its capabilities.

%\finding{For execution time and test number, \probdd and \proj perform
%comparable with each other, and are
%significant more superior than \ddmin.
%\victor{so what? I have this question for all insights and findings.}
%}

% size
\myparagraph{Effectiveness}
We assess the effectiveness by measuring the sizes of the final minimized
results.
 Our findings do not align with the claim in the original paper of \probdd, \ie,
 \probdd significantly
achieves a smaller average size than \ddmin. By contrast,
the effectiveness of \ddmin, \probdd and \proj varies across each
benchmark, but none of the algorithms consistently
outperforms the other two, substantiated by all the p-values of size
higher than
0.05.
%Our explanation is that, without domain specific information, any
%algorithm attempting to reduce a list of elements,
%may potentially get trapped in a local optimum, as test input minimization is
%an
%NP problem.
%On the uncompleted benchmarks, \probdd and \proj produce
%\benchmarkTimeoutSizeDecRateProbddVsDdmin and
%\benchmarkTimeoutSizeDecRateCddVsDdmin smaller size than \ddmin on
%the outputs, and \proj even achieves
%\benchmarkTimeoutSizeDecRateCddVsProbdd smaller than \probdd.
%However, based on unfinished benchmarks, we believe that such
%improvements indicate not a superiority in effectiveness, but rather in
%efficiency.

%\finding{\ddmin, \probdd and \proj show no
%significant differences in final size.}

% finding: similar size


% some special cases, such as string


==> evaluation/rq2.tex <==
%\input{table/rq2_test}
\finding{On tree-structured inputs, inefficient deletion
	attempts on complements
	and repeated
	attempts account for the bottleneck of \ddmin, which are overcome by
	\probdd and \proj.
}
\input{figure/rq2_distribution}

To further understand why \probdd and \proj are more efficient than
\ddmin, we
conduct in-depth statistics on the query number (number of deletion attempts).
Specifically,
%\victor{why can analyzing this help our understanding?}\mz{it helps to find
%out the bottleneck}
we classify the queries performed by \ddmin to
identify those with low success rates, revealing the
performance bottlenecks that impair \ddmin's efficiency but are
successfully
addressed by \probdd and \proj.

Specifically,
we categorize all the queries in \ddmin into three types, \ie,
\typeComplement, \typeRepeated and \typeOther. In
\picireny, reduction on each level starts with a sanity check query,
ensuring that \picireny operates correctly. For a more precise
comparison, we exclude such queries from the statistics.
\begin{enumerate}
	\item \typeComplement: Queries trying to remove the complement of a
	subset.
	According to \ddmin algorithm, given a
	subset (smaller than half of the list \listinput), it attempts to remove
	either the subset or its complement.
	However, evidence~\cite{hodovan2016practical} shows that keeping a
	small subset and
	removing its complement is not likely to succeed,
	especially on
	structured inputs such as programs and \xml files.
	\item \typeRepeated: Queries trying to remove the previously tried
	subset.
	After removing a subset, \ddmin restarts
	the process
	from the
	first subset, leading to repeated deletion attempts on previous subsets.
	\item \typeOther: All other queries.
\end{enumerate}
In addition to categorizing queries in \ddmin into the above types, we also
calculate the success rate of each type, aiming to reveal the
bottlenecks of \ddmin.
 \cref{fig:stacked_barchart} illustrates the distribution of queries for all
types within \ddmin, as well as the query number for \probdd and
\proj. We focus on \cBenchmarkNameShort
and
\xmlBenchmarkNameShort, as there is a significant
number of benchmarks
completed on both of them compared to the other two benchmark suites,
making the results
statistically meaningful.

On both \cBenchmarkNameShort and \xmlBenchmarkNameShort, \ddmin
performs almost the
same number of successful queries, compared to those of \probdd and
\proj. Specifically, on \cBenchmarkNameShort, \ddmin performs
$\cRepeatedNumberSuccessDdmin +
\cComplementNumberSuccessDdmin +
\cOtherNumberSuccessDdmin = \cSuccessNumberDdmin$ successful
queries, close to
\cSuccessNumberProbdd and \cSuccessNumberProj queries from \probdd
and \proj, respectively. Similarly, on \xmlBenchmarkNameShort, the success
query number of \ddmin is $\xmlRepeatedNumberSuccessDdmin +
\xmlComplementNumberSuccessDdmin +
\xmlOtherNumberSuccessDdmin = \xmlSuccessNumberDdmin$,
demonstrating only minimal
differences compared to
\probdd's \xmlSuccessNumberProbdd successful queries and \proj's
\xmlSuccessNumberProj successful queries. However, \ddmin performs
significantly more failed queries, resulting in a larger total
query number and thus a longer execution time, as discussed in
 \cref{sec:rq1}.

On both benchmark suites, a large portion of \ddmin's queries
is categorized as \typeComplement and \typeRepeated; however, they both
have a very low success rate. For instance, on
\cBenchmarkNameShort, out of a total of \cTotalNumberDdmin queries,
\typeComplement and \typeRepeated account for
\cComplementNumberDdmin (\cComplementPercentageDdmin) and
\cRepeatedNumberDdmin (\cRepeatedPercentageDdmin),
respectively. Within such queries in \typeComplement and \typeRepeated,
merely
\cComplementNumberSuccessDdmin (\cComplementSuccessRateDdmin)
and \cRepeatedNumberSuccessDdmin (\cRepeatedSuccessRateDdmin)
queries succeed, \ie, only a tiny portion of attempts
successfully reduce
elements. These success rates are far less than those of queries within
\typeOther (\cOtherSuccessRateDdmin), as well as those of \probdd
(\cSuccessRateProbdd) and
\proj (\cSuccessRateProj). On \xmlBenchmarkNameShort, a similar
phenomenon is observed.

Queries within \typeComplement and \typeRepeated categories constitute
a large portion yet prove to be largely inefficient,
 wasting a significant amount of time and resources. On the contrary,
 those in \typeOther achieve a much higher success rate, on par with that
 of \probdd and \proj, and
 are responsible for most of the successful deletions.
 Therefore, we
 believe that these two categories, where queries are inefficient, are
 the
 main bottlenecks
 behind \ddmin's low
 efficiency. However, these bottlenecks are absent in \probdd and \proj,
 as these two algorithms do not consider complements of subsets and
 previously tried subsets for deletion.

==> evaluation/rq3.tex <==
\finding{By comparing with \proj and \probddr,
	\probdd shows no significant improvement in performance. Therefore,
	element prioritization has no
	significant
	impact on the performance of \probdd.
}
\input{table/rq3_random}
As discussed in RQ1, \proj exhibits comparable performance
to \probdd in all aspects. However, \proj does not involve element
prioritization. Therefore, we speculate that
sorting elements by
probability in \probdd has no significant impact on the performance of
\probdd.
To further substantiate our hypothesis, we conduct an ablation study on
element prioritization via \probddr, a variant of \probdd. Specifically, to
disrupt
the ordering by \probdd, thereby
eliminating its influence, \probddr randomly shuffles the
elements before subset selection. As illustrated in
 \cref{table:rq3_random},
\probddr and \probdd have no significant differences \wrt size, execution
time and query number.

%\finding{Element sorting in \probdd has no significant impact to the
%performance.}

==> evaluation/rq4.tex <==
\finding{Improving efficiency by avoiding ineffective
	attempts
	presents a trade-off by not ensuring 1-minimality, while such limitation
	can be mitigated by iteratively running the reduction algorithm until a
	fixpoint is
	reached.}

Test input minimization is an NP problem,
signifying that no single algorithm can guarantee optimal results in every
scenario.
Evaluation on \stringBenchmarkNameShort showcases a limitation of \probdd
and \proj. As shown in
\cref{table:rq1_firsthalf} and \cref{table:rq1_secondhalf},
results produced by \probdd and \proj are always not
smaller than those from \ddmin. Across all benchmarks completed by every
algorithm, \ddmin
consistently achieved 1-minimality. However, neither \probdd nor \proj
achieves
1-minimal results on all benchmarks, as they avoid the attempts to delete
previously tried subsets, even though they might become removable
later.
 Specifically, \proj's result on \texttt{dc-1.3}
 included \mycode{["?", "[", "\textbackslash n"]}, where
 \mycode{"\textbackslash n"} is removable on its own.
Similarly, \probdd's outcome on \texttt{troff-1.19.2} retains
redundant characters
that could have been deleted.
Therefore, \probdd and \proj, by avoiding the deletion of
elements previously tried, might miss some reduction opportunities.

%\finding{Efficiency improvement can be achieved by avoiding repeated
%attempts, yet this approach does not guarantee 1-minimality, resulting in
%a
%trade-off.}

In contrast, such limitation is not apparent across the remaining three
benchmark suites, as the results from \probdd and \proj
are not
consistently larger than those from \ddmin. Our further investigation
reveals that these
benchmarks are about highly structured inputs, thereby being reduced on
wrapper frameworks
\picireny and \chisel. Both
frameworks employ iterative loops to achieve a fixpoint, effectively
reducing some elements missed in the first iteration.

%\researchquestion{\probdd and \proj do not guarantee to produce
%1-minimal results, while such limitation can be mitigated by iteratively
%running the algorithm until a fixpoint is reached.}


==> figure/bounds.tex <==
\begin{figure*}[t]
	\centering
%	\includegraphics[width=0.95\linewidth]{figure/bounds.pdf}
	\includegraphics[width=0.95\linewidth]{figure/bounds.pdf}

	\caption{
		The relationship between the size for next round $\mysize{r+1}{}$ and the
		size for
		current round $\mysize{r}{}$.
		The solid line represents
		$\mysize{r+1}{} = \frac{1}{ln(\frac{1 - e^{-1}}{e^{-\frac{1}{\mysize{r}{}}}-e^{-1}})}$,
		with the dashed lines representing its upper and lower bounds.
%		The enlarged portion represents the curve detail when size is close to 1.
%		The slope slightly changes when size is close to 1, but it does not
%affect the result as the size is always integer and the algorithm terminate
%at
%1.
%        \victor{this image is too large. Make it flatter and shorter}\mz{how about now?}
%        \cn{If you have time, remember to update the font in the pdf file.}
	  }
	\label{fig:bounds}


\end{figure*}

==> figure/rq2_figures.tex <==
\begin{figure}[htbp]
	\centering
	\begin{subfigure}{0.32\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figure/rq2_compilerbugs_size_boxplot.pdf}
		\caption{Size on }
		\label{fig:compiler_size}
	\end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/rq2_compilerbugs_test_boxplot.pdf}
        \caption{Query on }
        \label{fig:compiler_test}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/rq2_compilerbugs_time_boxplot.pdf}
        \caption{Time on }
        \label{fig:compiler_time}
    \end{subfigure}

	\begin{subfigure}{0.32\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figure/rq2_chisel_size_boxplot.pdf}
		\caption{Size on }
		\label{fig:chisel_size}
	\end{subfigure}
    \hfill
	\begin{subfigure}{0.32\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figure/rq2_chisel_test_boxplot.pdf}
		\caption{Query on }
		\label{fig:chisel_test}
	\end{subfigure}
    \hfill
	\begin{subfigure}{0.32\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figure/rq2_chisel_time_boxplot.pdf}
		\caption{Time on }
		\label{fig:chisel_time}
	\end{subfigure}

	\caption{Boxplots comparison among \ddmincos, \probdd, and \myalgorithm, as well as the p-values between each pair. \ddmincos denotes \ddmin with optimizations
    \complementonly (C), \onepass (O) and \myopt (S).
	}
	\label{fig:three_equivalent_variants}
\end{figure}






==> figure/rq3_figures.tex <==
\begin{figure*}[htbp]
	\centering
	\begin{subfigure}{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figure/rq3_compilerbugs_size_boxplot.pdf}
		\caption{Size on }
		\label{fig:compiler_size}
	\end{subfigure}
    \hfil
     \begin{subfigure}{0.45\textwidth}
    	\centering
    	\includegraphics[width=\textwidth]{figure/rq3_chisel_size_boxplot.pdf}
    	\caption{Size on }
    	\label{fig:chisel_size}
    \end{subfigure}


	\begin{subfigure}{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figure/rq3_compilerbugs_test_boxplot.pdf}
		\caption{Query on }
		\label{fig:compiler_test}
	\end{subfigure}
	\hfil
    \begin{subfigure}{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figure/rq3_chisel_test_boxplot.pdf}
		\caption{Query on }
		\label{fig:chisel_test}
	\end{subfigure}

	\begin{subfigure}{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figure/rq3_compilerbugs_time_boxplot.pdf}
		\caption{Time on }
		\label{fig:compiler_time}
	\end{subfigure}
	 \hfil
	\begin{subfigure}{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figure/rq3_chisel_time_boxplot.pdf}
		\caption{Time on }
		\label{fig:chisel_time}
	\end{subfigure}
	\caption{
		Transition from no optimization to 3 optimizations. To save space, we use subscripts instead of the full algorithm names. For example, we use C to represent \ddminc.
		From \ddmin, \complementonly (C), \onepass (O), and \myopt (S) are successively added, and several values (5-13) are evaluated as the threshold of \myopt. The red dashed line represents the mean value of \ddminco, which serves as the comparison baseline for all \myopt variations. The red cross marks display the mean values of other algorithms.
		Note that the range of test numbers has a large magnitude difference, so we use logarithmic scaling for better visualization.
	}
	\label{fig:different_thresholds}
\end{figure*}






==> futurework.tex <==
todo

\subsection{Partition size}



\subsection{Subtree size}

==> implications.tex <==

Findings 1,2,3 suggest that the probability can essentially be
optimized away from \probdd without impacting performance. Therefore, it
is not the
probability itself that is effective, but rather the \probdd algorithm's indirect
avoidance of certain bottlenecks. \textit{Consequently, for future research
in test
input minimization, despite the rising interest in probabilities and AI
models, deeper analyses such as ablation studies are essential to fully
ascertain the role and extent of model's effectiveness}.

According to Finding 4, the design of \probdd is more efficient than \ddmin
because it addresses inefficient queries related to the complements of
subsets and previously attempted subsets, which is effectively
summarized through categorization and visualization. \textit{Therefore, for
the design and evaluation
of test input minimization algorithms, the key is to visualize and identify
inefficient queries}.

As shown in Finding 5, the prioritization facilitated by \probdd does not
show a significant impact. However, some existing works introduce
effective element prioritization strategies, such as first removing usage
before declarations, or prioritizing deleting elements with no
dependencies~\cite{kalhauge2019binary, kalhauge2021logical}.
These approaches leverage domain knowledge to guarantee their
prioritization methods being effective. \textit{Therefore, future research
should ideally utilize domain
knowledge to ensure the effectiveness of prioritization. By contrast,
learning an
effective prioritization on the fly in a domain-agnostic scenario, like what
\probdd does,
faces greater challenges, thereby requiring more theoretical and empirical
support.}

Finding 6 indicates that a trade-off between effectiveness and efficiency
still exists within \probdd, requiring tailored decisions based on particular
scenarios.
On the other hand, \probdd avoids some inefficient queries,
which poses a risk of not achieving 1-minimality. However,
the fixpoint mechanism provided by \picireny, the wrapping framework,
ensures small enough final sizes and achieves greater efficiency when
using \probdd internally compared to \ddmin.
\textit{Therefore, the presence of trade-offs does not pessimistically imply
a lack
of optimization potential. Efficiently integrating the pivotal algorithms like
\probdd
and wrapping frameworks to
enhance performance is a promising research direction.}


==> lemmas/lem_lower_bound.tex <==
\begin{lem}
	The lower bound of $\mysize{r+1}{}$ w.r.t $\mysize{r}{}$ is

	\begin{align}
		\mysize{r+1}{} \ge (1 - e^{-1})\mysize{r}{}-1 \label{equation:lowerbound}
	\end{align}
	\label{lem:lower:bound}
\end{lem}

==> lemmas/lem_upper_bound.tex <==
\begin{lem}
	The upper bound of $\mysize{r+1}{}$ w.r.t $\mysize{r}{}$ is

	\begin{align}
		\mysize{r+1}{} \le (1 - e^{-1})\mysize{r}{} \label{equation:upperbound}
	\end{align}
	\label{lem:upper:bound}
\end{lem}

==> overview.tex <==
\cn{need to write an overview to introduce the structure of the paper.}
\cn{Let's finish this when we work on the introduction. We might not need this section, and include everything in
	the introduction.
}
\victor{is this done?}
\probdd has been demonstrated to
significantly improve reduction speed through its probabilistic model.
\cn{I am working on this paragraph.}
In the following,

However, \probdd consists of multiple steps, including element
prioritization, subset selection (as per \gain) and
probability
updates.
Despite its superior performance, the fundamental reason
has not been fully investigated.
Hence, we further analyze and refine the theory behind
\probdd, by applying appropriate mathematical derivation.


\victor{this section is so short?}\mz{do we need to remove this section? we
don't have enough space}
\cn{arg1}

==> table/probdd_vs_myalgorithm_init_p.tex <==
\begin{table}[]
	\centering
	\small
	\caption{
		Performance comparison of \probdd and \myalgorithm under different \pinit.
		The table shows the changes in the final program size, reduction time, and test number for \myalgorithm relative to \probdd, given \pinit being 0.05, 0.1, 0.15, 0.2, and 0.25.
		For each \pinit initial value, there are two columns corresponding.
		The first column shows the average percentage difference of \myalgorithm compared to \probdd,
		and the second column presents the p-value, indicating the significance of such difference.
	}
	\label{table:probdd_vs_myalgorithm_init_p}
	\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}c|rr|rr|rr|rr|rr@{}}
	\toprule
	Initial probability & \multicolumn{2}{c|}{0.05} & \multicolumn{2}{c|}{0.1} & \multicolumn{2}{c|}{0.15} & \multicolumn{2}{c|}{0.2} & \multicolumn{2}{c}{0.25} \\ \midrule
	Final size (\#)     & 0.59\%       & 0.1704      & -1.08\%      & 0.1467     & 0.84\%        & 0.1892     & -0.79\%      & 0.2515     & 0.10\%       & 0.7299     \\
	Time (h)            & 8.01\%       & 0.3083      & -11.05\%     & \textbf{0.0240}     & -5.06\%       & 0.0874     & 0.98\%       & 0.8939     & -13.21\%     & 0.2943     \\
	Query number (\#)   & 5.12\%       & 0.6087      & -14.56\%     & \textbf{0.0286}     & -18.58\%      & \textbf{0.0002}     & -13.18\%     & 0.0927     & -28.91\%     & 0.0850     \\ \bottomrule
\end{tabular}
	}
\end{table}


==> table/probdd_vs_myalgorithm_size.tex <==
\begin{table}[]
	\centering
	\caption{The reduction size comparison between \ddmin, \probdd and
	\proj on xxx benchmarks.
		We calculated the mean values, reduction ratio for all algorithms. We also conducted a paired sample t-test
		between these algorithms in pairs and computed their p-values.
%        \cn{The sizes are not great.}\mz{done}
	}
	\label{table:probdd_vs_myalgorithm_size}
%\resizebox{\linewidth}{!}{%
%    \renewcommand{\arraystretch}{0.95}
\begin{tabular}{@{}c|r|rrr@{}}
	\toprule
	& \multicolumn{1}{c|}{}                                     & \multicolumn{3}{c}{Final size (\#)}                                                                                                         \\ \cmidrule(l){3-5}
	\multirow{-2}{*}{Benchmark} & \multicolumn{1}{c|}{\multirow{-2}{*}{Original size (\#)}} & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\ddmin} & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}\probdd} & \multicolumn{1}{c}{\myalgorithm} \\ \midrule
	\llvm-22382                 & 9,987                                                     & \cellcolor[HTML]{C0C0C0}351                        & \cellcolor[HTML]{EFEFEF}351                         & 351                              \\
	\llvm-22704                 & 184,444                                                   & \cellcolor[HTML]{C0C0C0}785                        & \cellcolor[HTML]{EFEFEF}785                         & 789                              \\
	\llvm-23309                 & 33,310                                                    & \cellcolor[HTML]{C0C0C0}410                        & \cellcolor[HTML]{EFEFEF}815                         & 320                              \\
	\llvm-23353                 & 30,196                                                    & \cellcolor[HTML]{C0C0C0}344                        & \cellcolor[HTML]{EFEFEF}325                         & 325                              \\
	\llvm-25900                 & 78,960                                                    & \cellcolor[HTML]{C0C0C0}912                        & \cellcolor[HTML]{EFEFEF}911                         & 908                              \\
	\llvm-26760                 & 209,577                                                   & \cellcolor[HTML]{C0C0C0}521                        & \cellcolor[HTML]{EFEFEF}513                         & 521                              \\
	\llvm-27137                 & 174,538                                                   & \cellcolor[HTML]{C0C0C0}288                        & \cellcolor[HTML]{EFEFEF}222                         & 222                              \\
	\llvm-27747                 & 173,840                                                   & \cellcolor[HTML]{C0C0C0}424                        & \cellcolor[HTML]{EFEFEF}424                         & 424                              \\
	\llvm-31259                 & 48,799                                                    & \cellcolor[HTML]{C0C0C0}1,023                      & \cellcolor[HTML]{EFEFEF}836                         & 838                              \\
	\gcc-59903                  & 57,581                                                    & \cellcolor[HTML]{C0C0C0}1,156                      & \cellcolor[HTML]{EFEFEF}1,204                       & 723                              \\
	\gcc-60116                  & 75,224                                                    & \cellcolor[HTML]{C0C0C0}355                        & \cellcolor[HTML]{EFEFEF}359                         & 370                              \\
	\gcc-61383                  & 32,449                                                    & \cellcolor[HTML]{C0C0C0}939                        & \cellcolor[HTML]{EFEFEF}915                         & 939                              \\
	\gcc-61917                   & 85,359                                                    & \cellcolor[HTML]{C0C0C0}863                        & \cellcolor[HTML]{EFEFEF}897                         & 879                              \\
	\gcc-64990                  & 148,931                                                   & \cellcolor[HTML]{C0C0C0}737                        & \cellcolor[HTML]{EFEFEF}711                         & 712                              \\
	\gcc-65383                  & 43,942                                                    & \cellcolor[HTML]{C0C0C0}663                        & \cellcolor[HTML]{EFEFEF}650                         & 663                              \\
	\gcc-66186                  & 47,481                                                    & \cellcolor[HTML]{C0C0C0}971                        & \cellcolor[HTML]{EFEFEF}973                         & 971                              \\
	\gcc-66375                  & 65,488                                                    & \cellcolor[HTML]{C0C0C0}454                        & \cellcolor[HTML]{EFEFEF}908                         & 451                              \\
	\gcc-70127                  & 154,816                                                   & \cellcolor[HTML]{C0C0C0}342                        & \cellcolor[HTML]{EFEFEF}211                         & 211                              \\
	\gcc-70586                  & 212,259                                                   & \cellcolor[HTML]{C0C0C0}1,469                      & \cellcolor[HTML]{EFEFEF}1,493                       & 1,476                            \\
	\gcc-71626                  & 4,397                                                     & \cellcolor[HTML]{C0C0C0}179                        & \cellcolor[HTML]{EFEFEF}179                         & 179                              \\
	bzip2-1.0.5                 & 70,530                                                    & \cellcolor[HTML]{C0C0C0}20,703                     & \cellcolor[HTML]{EFEFEF}20,707                      & 20,756                           \\
	chown-8.2                   & 43,869                                                    & \cellcolor[HTML]{C0C0C0}9,163                      & \cellcolor[HTML]{EFEFEF}9,253                       & 9,269                            \\
	date-8.21                   & 53,442                                                    & \cellcolor[HTML]{C0C0C0}33,033                     & \cellcolor[HTML]{EFEFEF}20,782                      & 20,616                           \\
	grep-2.19                   & 127,681                                                   & \cellcolor[HTML]{C0C0C0}23,996                     & \cellcolor[HTML]{EFEFEF}29,697                      & 28,789                           \\
	gzip-1.2.4                  & 45,929                                                    & \cellcolor[HTML]{C0C0C0}17,055                     & \cellcolor[HTML]{EFEFEF}17,057                      & 17,241                           \\
	mkdir-5.2.1                 & 34,801                                                    & \cellcolor[HTML]{C0C0C0}8,625                      & \cellcolor[HTML]{EFEFEF}8,407                       & 8,407                            \\
	rm-8.4                      & 44,459                                                    & \cellcolor[HTML]{C0C0C0}8,520                      & \cellcolor[HTML]{EFEFEF}8,414                       & 8,436                            \\
	sort-8.16                   & 88,068                                                    & \cellcolor[HTML]{C0C0C0}14,935                     & \cellcolor[HTML]{EFEFEF}14,871                      & 15,226                           \\
	tar-1.14                    & 163,296                                                   & \cellcolor[HTML]{C0C0C0}20,061                     & \cellcolor[HTML]{EFEFEF}20,423                      & 20,506                           \\
	uniq-8.16                   & 63,861                                                    & \cellcolor[HTML]{C0C0C0}14,350                     & \cellcolor[HTML]{EFEFEF}14,354                      & 14,206                           \\ \midrule
	Average   Size                  & 73,594                                                    & \cellcolor[HTML]{C0C0C0}6,121                      & \cellcolor[HTML]{EFEFEF}5,922                       & 5,857                            \\
	Average Reduction ratio             &                                                           & \cellcolor[HTML]{C0C0C0}91.68\%                     & \cellcolor[HTML]{EFEFEF}91.95\%                      & 92.04\%                           \\
	p-value to \ddmin           &                                                           & \cellcolor[HTML]{C0C0C0}                           & \cellcolor[HTML]{EFEFEF}0.6662                      & 0.5623                           \\
	p-value to \probdd          &                                                           & \cellcolor[HTML]{C0C0C0}                           & \cellcolor[HTML]{EFEFEF}                            & 0.1467                           \\ \bottomrule
\end{tabular}
%}
\end{table}


==> table/probdd_vs_myalgorithm_time.tex <==
\begin{table}[]
	\centering
	\caption{The reduction time and test number comparison between \ddmin, \probdd and \myalgorithm.
		We calculated the mean values of time and test number, and conducted paired sample t-test.
%        \cn{Why do we use hours here. At least you should use HH:mm:ss, or minutes.}\mz{done}
	}
	\label{table:probdd_vs_myalgorithm_time}
%\resizebox{\linewidth}{!}{%
%    \renewcommand{\arraystretch}{0.95}
\begin{tabular}{@{}c|rrr|rrr@{}}
	\toprule
	& \multicolumn{3}{c|}{Time (hh:mm:ss)}                                                                                                                & \multicolumn{3}{c}{Query number (\#)}                                                                                                       \\ \cmidrule(l){2-7}
	\multirow{-2}{*}{Benchmark} & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\ddmin} & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}\probdd} & \multicolumn{1}{c|}{\myalgorithm} & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\ddmin} & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}\probdd} & \multicolumn{1}{c}{\myalgorithm} \\ \midrule
	\llvm-22382                 & \cellcolor[HTML]{C0C0C0}0:14:17                    & \cellcolor[HTML]{EFEFEF}0:10:29                     & 0:08:56                           & \cellcolor[HTML]{C0C0C0}10,643                     & \cellcolor[HTML]{EFEFEF}5,046                       & 4,039                            \\
	\llvm-22704                 & \cellcolor[HTML]{C0C0C0}4:43:03                    & \cellcolor[HTML]{EFEFEF}2:29:55                     & 2:34:27                           & \cellcolor[HTML]{C0C0C0}50,340                     & \cellcolor[HTML]{EFEFEF}11,479                      & 10,880                           \\
	\llvm-23309                 & \cellcolor[HTML]{C0C0C0}2:04:03                    & \cellcolor[HTML]{EFEFEF}2:05:38                     & 0:43:13                           & \cellcolor[HTML]{C0C0C0}41,079                     & \cellcolor[HTML]{EFEFEF}20,234                      & 7,927                            \\
	\llvm-23353                 & \cellcolor[HTML]{C0C0C0}0:20:15                    & \cellcolor[HTML]{EFEFEF}0:12:26                     & 0:11:22                           & \cellcolor[HTML]{C0C0C0}10,440                     & \cellcolor[HTML]{EFEFEF}3,188                       & 2,626                            \\
	\llvm-25900                 & \cellcolor[HTML]{C0C0C0}1:17:01                    & \cellcolor[HTML]{EFEFEF}0:41:06                     & 0:39:37                           & \cellcolor[HTML]{C0C0C0}33,761                     & \cellcolor[HTML]{EFEFEF}8,168                       & 8,857                            \\
	\llvm-26760                 & \cellcolor[HTML]{C0C0C0}1:26:51                    & \cellcolor[HTML]{EFEFEF}0:50:33                     & 0:43:49                           & \cellcolor[HTML]{C0C0C0}26,484                     & \cellcolor[HTML]{EFEFEF}7,690                       & 5,870                            \\
	\llvm-27137                 & \cellcolor[HTML]{C0C0C0}12:45:37                   & \cellcolor[HTML]{EFEFEF}4:09:33                     & 3:41:49                           & \cellcolor[HTML]{C0C0C0}106,669                    & \cellcolor[HTML]{EFEFEF}13,418                      & 11,530                           \\
	\llvm-27747                 & \cellcolor[HTML]{C0C0C0}0:53:25                    & \cellcolor[HTML]{EFEFEF}0:38:07                     & 0:35:34                           & \cellcolor[HTML]{C0C0C0}18,532                     & \cellcolor[HTML]{EFEFEF}6,295                       & 5,401                            \\
	\llvm-31259                 & \cellcolor[HTML]{C0C0C0}2:17:48                    & \cellcolor[HTML]{EFEFEF}1:09:56                     & 0:58:58                           & \cellcolor[HTML]{C0C0C0}37,982                     & \cellcolor[HTML]{EFEFEF}9,077                       & 7,707                            \\
	\gcc-59903                  & \cellcolor[HTML]{C0C0C0}1:30:58                    & \cellcolor[HTML]{EFEFEF}1:02:53                     & 0:51:34                           & \cellcolor[HTML]{C0C0C0}45,647                     & \cellcolor[HTML]{EFEFEF}14,298                      & 10,328                           \\
	\gcc-60116                  & \cellcolor[HTML]{C0C0C0}7:04:04                    & \cellcolor[HTML]{EFEFEF}2:05:24                     & 1:36:26                           & \cellcolor[HTML]{C0C0C0}49,612                     & \cellcolor[HTML]{EFEFEF}10,268                      & 8,304                            \\
	\gcc-61383                  & \cellcolor[HTML]{C0C0C0}1:52:27                    & \cellcolor[HTML]{EFEFEF}1:12:06                     & 0:49:16                           & \cellcolor[HTML]{C0C0C0}41,739                     & \cellcolor[HTML]{EFEFEF}15,044                      & 9,538                            \\
	\gcc-61917                   & \cellcolor[HTML]{C0C0C0}1:02:06                    & \cellcolor[HTML]{EFEFEF}0:32:01                     & 0:28:53                           & \cellcolor[HTML]{C0C0C0}28,512                     & \cellcolor[HTML]{EFEFEF}9,450                       & 7,881                            \\
	\gcc-64990                  & \cellcolor[HTML]{C0C0C0}3:26:46                    & \cellcolor[HTML]{EFEFEF}1:58:55                     & 1:44:57                           & \cellcolor[HTML]{C0C0C0}42,749                     & \cellcolor[HTML]{EFEFEF}11,014                      & 9,810                            \\
	\gcc-65383                  & \cellcolor[HTML]{C0C0C0}0:58:55                    & \cellcolor[HTML]{EFEFEF}0:34:04                     & 0:30:07                           & \cellcolor[HTML]{C0C0C0}26,235                     & \cellcolor[HTML]{EFEFEF}7,356                       & 6,306                            \\
	\gcc-66186                  & \cellcolor[HTML]{C0C0C0}1:25:05                    & \cellcolor[HTML]{EFEFEF}0:54:07                     & 0:42:00                           & \cellcolor[HTML]{C0C0C0}38,746                     & \cellcolor[HTML]{EFEFEF}13,338                      & 9,028                            \\
	\gcc-66375                  & \cellcolor[HTML]{C0C0C0}1:30:14                    & \cellcolor[HTML]{EFEFEF}1:09:59                     & 0:40:47                           & \cellcolor[HTML]{C0C0C0}37,933                     & \cellcolor[HTML]{EFEFEF}16,853                      & 8,906                            \\
	\gcc-70127                  & \cellcolor[HTML]{C0C0C0}2:19:32                    & \cellcolor[HTML]{EFEFEF}1:07:44                     & 0:59:32                           & \cellcolor[HTML]{C0C0C0}43,734                     & \cellcolor[HTML]{EFEFEF}10,196                      & 8,819                            \\
	\gcc-70586                  & \cellcolor[HTML]{C0C0C0}6:35:02                    & \cellcolor[HTML]{EFEFEF}3:28:26                     & 2:24:19                           & \cellcolor[HTML]{C0C0C0}88,583                     & \cellcolor[HTML]{EFEFEF}21,569                      & 16,185                           \\
	\gcc-71626                  & \cellcolor[HTML]{C0C0C0}0:01:21                    & \cellcolor[HTML]{EFEFEF}0:01:09                     & 0:01:09                           & \cellcolor[HTML]{C0C0C0}1,520                      & \cellcolor[HTML]{EFEFEF}1,125                       & 898                              \\
	bzip2-1.0.5                 & \cellcolor[HTML]{C0C0C0}40:04:55                   & \cellcolor[HTML]{EFEFEF}30:19:02                    & 25:46:47                          & \cellcolor[HTML]{C0C0C0}54,030                     & \cellcolor[HTML]{EFEFEF}25,142                      & 17,324                           \\
	chown-8.2                   & \cellcolor[HTML]{C0C0C0}5:17:59                    & \cellcolor[HTML]{EFEFEF}1:47:21                     & 1:51:56                           & \cellcolor[HTML]{C0C0C0}44,336                     & \cellcolor[HTML]{EFEFEF}5,518                       & 5,334                            \\
	date-8.21                   & \cellcolor[HTML]{C0C0C0}12:32:09                   & \cellcolor[HTML]{EFEFEF}5:07:03                     & 5:13:51                           & \cellcolor[HTML]{C0C0C0}98,799                     & \cellcolor[HTML]{EFEFEF}14,226                      & 13,718                           \\
	grep-2.19                   & \cellcolor[HTML]{C0C0C0}40:46:06                   & \cellcolor[HTML]{EFEFEF}28:08:45                    & 25:56:39                          & \cellcolor[HTML]{C0C0C0}289,249                    & \cellcolor[HTML]{EFEFEF}28,959                      & 38,547                           \\
	gzip-1.2.4                  & \cellcolor[HTML]{C0C0C0}15:07:36                   & \cellcolor[HTML]{EFEFEF}7:37:15                     & 8:38:22                           & \cellcolor[HTML]{C0C0C0}94,160                     & \cellcolor[HTML]{EFEFEF}17,466                      & 23,250                           \\
	mkdir-5.2.1                 & \cellcolor[HTML]{C0C0C0}1:08:06                    & \cellcolor[HTML]{EFEFEF}0:37:54                     & 0:34:24                           & \cellcolor[HTML]{C0C0C0}11,968                     & \cellcolor[HTML]{EFEFEF}2,468                       & 1,855                            \\
	rm-8.4                      & \cellcolor[HTML]{C0C0C0}3:52:04                    & \cellcolor[HTML]{EFEFEF}1:20:44                     & 1:18:34                           & \cellcolor[HTML]{C0C0C0}33,532                     & \cellcolor[HTML]{EFEFEF}4,976                       & 4,834                            \\
	sort-8.16                   & \cellcolor[HTML]{C0C0C0}17:46:31                   & \cellcolor[HTML]{EFEFEF}14:19:04                    & 14:31:28                          & \cellcolor[HTML]{C0C0C0}88,291                     & \cellcolor[HTML]{EFEFEF}9,560                       & 10,459                           \\
	tar-1.14                    & \cellcolor[HTML]{C0C0C0}29:54:41                   & \cellcolor[HTML]{EFEFEF}10:33:28                    & 7:14:37                           & \cellcolor[HTML]{C0C0C0}219,565                    & \cellcolor[HTML]{EFEFEF}10,588                      & 9,282                            \\
	uniq-8.16                   & \cellcolor[HTML]{C0C0C0}4:27:10                    & \cellcolor[HTML]{EFEFEF}2:56:03                     & 2:50:17                           & \cellcolor[HTML]{C0C0C0}25,885                     & \cellcolor[HTML]{EFEFEF}3,797                       & 3,193                            \\ \midrule
	Average                     & \cellcolor[HTML]{C0C0C0}7:29:32                    & \cellcolor[HTML]{EFEFEF}4:18:42                     & 3:50:07                           & \cellcolor[HTML]{C0C0C0}58,025                     & \cellcolor[HTML]{EFEFEF}11,260                      & 9,621                            \\
	Decrease relative to \ddmin & \cellcolor[HTML]{C0C0C0}                           & \cellcolor[HTML]{EFEFEF}-42.45\%                     & -48.81\%                           & \cellcolor[HTML]{C0C0C0}                           & \cellcolor[HTML]{EFEFEF}-80.59\%                     & -83.42\%                          \\
	p-value to \ddmin           & \cellcolor[HTML]{C0C0C0}                           & \cellcolor[HTML]{EFEFEF}5.9E-04                     & 7.1E-04                           & \cellcolor[HTML]{C0C0C0}                           & \cellcolor[HTML]{EFEFEF}9.6E-05                     & 4.1E-05                          \\
	p-value to \probdd          & \cellcolor[HTML]{C0C0C0}                           & \cellcolor[HTML]{EFEFEF}                            & 0.0240                            & \cellcolor[HTML]{C0C0C0}                           & \cellcolor[HTML]{EFEFEF}                            & 0.0286                           \\ \bottomrule
\end{tabular}
%}
\end{table}


==> table/rq1_all.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[]
		\centering
		\footnotesize
	\caption{The final size, execution time and query number of
		\ddmin, \probdd and
		\proj on all benchmark suites.
		To address significant variations across benchmarks, the geometric
		mean rather than the arithmetic mean is employed, providing a
		smoother measure of the average.
	}
	\label{table:rq1_all}
	\resizebox{0.85\linewidth}{!}{%
\begin{tabular}{c|l|r|rrr|rrr|rrr}
	\toprule
	\multicolumn{1}{l|}{}                         & \multicolumn{1}{c|}{}
	& \multicolumn{1}{c|}{}                                     & \multicolumn{3}{c|}{Final
	size (\#)}                                                                                              &
	\multicolumn{3}{c|}{Execution time
	(s)}                                                                                           &
	\multicolumn{3}{c}{Query
	number}                                                                                                 \\
	\cmidrule(l){4-12}
	\multicolumn{1}{l|}{\multirow{-2}{*}{}}       &
	\multicolumn{1}{c|}{\multirow{-2}{*}{Benchmark}} &
	\multicolumn{1}{c|}{\multirow{-2}{*}{Original size (\#)}} &
	\multicolumn{1}{c}{\cellcolor[HTML]{B7B7B7}ddmin} &
	\multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}ProbDD} &
	\multicolumn{1}{c|}{CDD} &
	\multicolumn{1}{c}{\cellcolor[HTML]{B7B7B7}ddmin} &
	\multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}ProbDD} &
	\multicolumn{1}{c|}{CDD} &
	\multicolumn{1}{c}{\cellcolor[HTML]{B7B7B7}ddmin} &
	\multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}ProbDD} &
	\multicolumn{1}{c}{CDD} \\ \midrule
	& \llvm-22382                                      &
	9,987                                                     &
	\cellcolor[HTML]{B7B7B7}350                       &
	\cellcolor[HTML]{EFEFEF}353                        & 350                      &
	\cellcolor[HTML]{B7B7B7}1,917                     &
	\cellcolor[HTML]{EFEFEF}1,163                      & 1,005                    &
	\cellcolor[HTML]{B7B7B7}11,388                    &
	\cellcolor[HTML]{EFEFEF}5,973                      & 5,262                   \\
	& \llvm-22704                                      &
	184,444                                                   &
	\cellcolor[HTML]{B7B7B7}786                       &
	\cellcolor[HTML]{EFEFEF}764                        & 745                      &
	\cellcolor[HTML]{B7B7B7}27,924                    &
	\cellcolor[HTML]{EFEFEF}12,418                     & 11,371                   &
	\cellcolor[HTML]{B7B7B7}52,412                    &
	\cellcolor[HTML]{EFEFEF}15,425                     & 14,025                  \\
	& \llvm-23309                                      &
	33,310                                                    &
	\cellcolor[HTML]{B7B7B7}1,316                     &
	\cellcolor[HTML]{EFEFEF}1,338                      & 1,265                    &
	\cellcolor[HTML]{B7B7B7}17,619                    &
	\cellcolor[HTML]{EFEFEF}9,991                      & 10,828                   &
	\cellcolor[HTML]{B7B7B7}55,968                    &
	\cellcolor[HTML]{EFEFEF}19,195                     & 17,953                  \\
	& \llvm-23353                                      &
	30,196                                                    &
	\cellcolor[HTML]{B7B7B7}321                       &
	\cellcolor[HTML]{EFEFEF}336                        & 324                      &
	\cellcolor[HTML]{B7B7B7}3,117                     &
	\cellcolor[HTML]{EFEFEF}1,874                      & 1,400                    &
	\cellcolor[HTML]{B7B7B7}11,719                    &
	\cellcolor[HTML]{EFEFEF}5,757                      & 4,492                   \\
	& \llvm-25900                                      &
	78,960                                                    &
	\cellcolor[HTML]{B7B7B7}941                       &
	\cellcolor[HTML]{EFEFEF}932                        & 937                      &
	\cellcolor[HTML]{B7B7B7}7,258                     &
	\cellcolor[HTML]{EFEFEF}3,683                      & 3,104                    &
	\cellcolor[HTML]{B7B7B7}35,740                    &
	\cellcolor[HTML]{EFEFEF}12,553                     & 12,817                  \\
	& \llvm-26760                                      &
	209,577                                                   &
	\cellcolor[HTML]{B7B7B7}520                       &
	\cellcolor[HTML]{EFEFEF}503                        & 498                      &
	\cellcolor[HTML]{B7B7B7}13,123                    &
	\cellcolor[HTML]{EFEFEF}5,876                      & 5,210                    &
	\cellcolor[HTML]{B7B7B7}30,063                    &
	\cellcolor[HTML]{EFEFEF}9,261                      & 9,792                   \\
	& \llvm-27137                                      &
	174,538                                                   &
	\cellcolor[HTML]{B7B7B7}972                       &
	\cellcolor[HTML]{EFEFEF}1,040                      & 966                      &
	\cellcolor[HTML]{B7B7B7}63,971                    &
	\cellcolor[HTML]{EFEFEF}22,208                     & 23,154                   &
	\cellcolor[HTML]{B7B7B7}122,516                   &
	\cellcolor[HTML]{EFEFEF}22,292                     & 20,460                  \\
	& \llvm-27747                                      &
	173,840                                                   &
	\cellcolor[HTML]{B7B7B7}431                       &
	\cellcolor[HTML]{EFEFEF}463                        & 510                      &
	\cellcolor[HTML]{B7B7B7}6,545                     &
	\cellcolor[HTML]{EFEFEF}4,238                      & 2,932                    &
	\cellcolor[HTML]{B7B7B7}20,000                    &
	\cellcolor[HTML]{EFEFEF}8,193                      & 5,992                   \\
	& \llvm-31259                                      &
	48,799                                                    &
	\cellcolor[HTML]{B7B7B7}1,033                     &
	\cellcolor[HTML]{EFEFEF}965                        & 1,035                    &
	\cellcolor[HTML]{B7B7B7}13,815                    &
	\cellcolor[HTML]{EFEFEF}7,497                      & 8,205                    &
	\cellcolor[HTML]{B7B7B7}35,135                    &
	\cellcolor[HTML]{EFEFEF}10,776                     & 13,445                  \\
	& \gcc-59903                                       &
	57,581                                                    &
	\cellcolor[HTML]{B7B7B7}1,185                     &
	\cellcolor[HTML]{EFEFEF}845                        & 743                      &
	\cellcolor[HTML]{B7B7B7}9,067                     &
	\cellcolor[HTML]{EFEFEF}4,879                      & 3,587                    &
	\cellcolor[HTML]{B7B7B7}47,698                    &
	\cellcolor[HTML]{EFEFEF}15,725                     & 13,844                  \\
	& \gcc-60116                                       &
	75,224                                                    &
	\cellcolor[HTML]{B7B7B7}1,615                     &
	\cellcolor[HTML]{EFEFEF}1,628                      & 1,617                    &
	\cellcolor[HTML]{B7B7B7}44,287                    &
	\cellcolor[HTML]{EFEFEF}27,202                     & 27,195                   &
	\cellcolor[HTML]{B7B7B7}80,059                    &
	\cellcolor[HTML]{EFEFEF}27,268                     & 23,204                  \\
	& \gcc-61383                                       &
	32,449                                                    &
	\cellcolor[HTML]{B7B7B7}959                       &
	\cellcolor[HTML]{EFEFEF}966                        & 974                      &
	\cellcolor[HTML]{B7B7B7}12,579                    &
	\cellcolor[HTML]{EFEFEF}6,514                      & 6,566                    &
	\cellcolor[HTML]{B7B7B7}43,716                    &
	\cellcolor[HTML]{EFEFEF}13,593                     & 14,149                  \\
	& \gcc-61917                                       &
	85,359                                                    &
	\cellcolor[HTML]{B7B7B7}882                       &
	\cellcolor[HTML]{EFEFEF}908                        & 884                      &
	\cellcolor[HTML]{B7B7B7}6,740                     &
	\cellcolor[HTML]{EFEFEF}3,591                      & 2,953                    &
	\cellcolor[HTML]{B7B7B7}31,414                    &
	\cellcolor[HTML]{EFEFEF}12,908                     & 14,194                  \\
	& \gcc-64990                                       &
	148,931                                                   &
	\cellcolor[HTML]{B7B7B7}744                       &
	\cellcolor[HTML]{EFEFEF}876                        & 681                      &
	\cellcolor[HTML]{B7B7B7}21,633                    &
	\cellcolor[HTML]{EFEFEF}11,890                     & 11,119                   &
	\cellcolor[HTML]{B7B7B7}44,521                    &
	\cellcolor[HTML]{EFEFEF}16,074                     & 12,112                  \\
	& \gcc-65383                                       &
	43,942                                                    &
	\cellcolor[HTML]{B7B7B7}706                       &
	\cellcolor[HTML]{EFEFEF}701                        & 709                      &
	\cellcolor[HTML]{B7B7B7}5,132                     &
	\cellcolor[HTML]{EFEFEF}3,543                      & 3,358                    &
	\cellcolor[HTML]{B7B7B7}25,051                    &
	\cellcolor[HTML]{EFEFEF}8,591                      & 9,686                   \\
	& \gcc-66186                                       &
	47,481                                                    &
	\cellcolor[HTML]{B7B7B7}1,012                     &
	\cellcolor[HTML]{EFEFEF}981                        & 1,001                    &
	\cellcolor[HTML]{B7B7B7}14,280                    &
	\cellcolor[HTML]{EFEFEF}7,236                      & 12,478                   &
	\cellcolor[HTML]{B7B7B7}47,253                    &
	\cellcolor[HTML]{EFEFEF}12,741                     & 19,094                  \\
	& \gcc-66375                                       &
	65,488                                                    &
	\cellcolor[HTML]{B7B7B7}1,128                     &
	\cellcolor[HTML]{EFEFEF}1,141                      & 1,204                    &
	\cellcolor[HTML]{B7B7B7}23,576                    &
	\cellcolor[HTML]{EFEFEF}14,182                     & 23,229                   &
	\cellcolor[HTML]{B7B7B7}47,339                    &
	\cellcolor[HTML]{EFEFEF}15,690                     & 16,469                  \\
	& \gcc-70127                                       &
	154,816                                                   &
	\cellcolor[HTML]{B7B7B7}934                       &
	\cellcolor[HTML]{EFEFEF}973                        & 930                      &
	\cellcolor[HTML]{B7B7B7}36,390                    &
	\cellcolor[HTML]{EFEFEF}23,925                     & 24,143                   &
	\cellcolor[HTML]{B7B7B7}54,925                    &
	\cellcolor[HTML]{EFEFEF}15,388                     & 15,219                  \\
	& \gcc-70586                                       &
	212,259                                                   &
	\cellcolor[HTML]{B7B7B7}1,583                     &
	\cellcolor[HTML]{EFEFEF}1,561                      & 1,572                    &
	\cellcolor[HTML]{B7B7B7}28,859                    &
	\cellcolor[HTML]{EFEFEF}13,519                     & 15,818                   &
	\cellcolor[HTML]{B7B7B7}102,603                   &
	\cellcolor[HTML]{EFEFEF}24,716                     & 30,715                  \\
	& \gcc-71626                                       &
	4,397                                                     &
	\cellcolor[HTML]{B7B7B7}184                       &
	\cellcolor[HTML]{EFEFEF}184                        & 184                      &
	\cellcolor[HTML]{B7B7B7}119                       &
	\cellcolor[HTML]{EFEFEF}114                        & 99                       &
	\cellcolor[HTML]{B7B7B7}1,608                     &
	\cellcolor[HTML]{EFEFEF}1,156                      & 1,220                   \\
	\cmidrule(l){2-12}
	\multirow{-21}{*}{\cBenchmarkNameShort}       &
	\multicolumn{1}{c|}{Mean}                        &
	64,599                                                    &
	\cellcolor[HTML]{B7B7B7}777                       &
	\cellcolor[HTML]{EFEFEF}775                        & 760                      &
	\cellcolor[HTML]{B7B7B7}10,486                    &
	\cellcolor[HTML]{EFEFEF}5,828                      & 5,676                    &
	\cellcolor[HTML]{B7B7B7}34,013                    &
	\cellcolor[HTML]{EFEFEF}11,652                     & 11,512                  \\ \midrule
	& bzip2-1.0.5                                      &
	70,530                                                    &
	\cellcolor[HTML]{B7B7B7}20,710                    &
	\cellcolor[HTML]{EFEFEF}20,747                     & 20,756                   &
	\cellcolor[HTML]{B7B7B7}137,463                   &
	\cellcolor[HTML]{EFEFEF}105,782                    & 92,058                   &
	\cellcolor[HTML]{B7B7B7}54,034                    &
	\cellcolor[HTML]{EFEFEF}23,240                     & 19,846                  \\
	& chown-8.2                                        &
	43,869                                                    &
	\cellcolor[HTML]{B7B7B7}9,087                     &
	\cellcolor[HTML]{EFEFEF}9,303                      & 9,310                    &
	\cellcolor[HTML]{B7B7B7}38,902                    &
	\cellcolor[HTML]{EFEFEF}25,616                     & 7,625                    &
	\cellcolor[HTML]{B7B7B7}50,487                    &
	\cellcolor[HTML]{EFEFEF}8,278                      & 8,208                   \\
	& date-8.21                                        &
	53,442                                                    &
	\cellcolor[HTML]{B7B7B7}20,604                    &
	\cellcolor[HTML]{EFEFEF}20,738                     & 21,120                   &
	\cellcolor[HTML]{B7B7B7}115,292                   &
	\cellcolor[HTML]{EFEFEF}16,486                     & 15,378                   &
	\cellcolor[HTML]{B7B7B7}139,934                   &
	\cellcolor[HTML]{EFEFEF}14,235                     & 13,928                  \\
	& grep-2.19                                        &
	127,681                                                   &
	\cellcolor[HTML]{B7B7B7}28,723                    &
	\cellcolor[HTML]{EFEFEF}28,627                     & 28,990                   &
	\cellcolor[HTML]{B7B7B7}97,821                    &
	\cellcolor[HTML]{EFEFEF}85,694                     & 93,552                   &
	\cellcolor[HTML]{B7B7B7}277,130                   &
	\cellcolor[HTML]{EFEFEF}42,246                     & 37,607                  \\
	& gzip-1.2.4                                       &
	45,929                                                    &
	\cellcolor[HTML]{B7B7B7}17,065                    &
	\cellcolor[HTML]{EFEFEF}17,068                     & 17,077                   &
	\cellcolor[HTML]{B7B7B7}73,403                    &
	\cellcolor[HTML]{EFEFEF}55,520                     & 75,913                   &
	\cellcolor[HTML]{B7B7B7}147,035                   &
	\cellcolor[HTML]{EFEFEF}27,569                     & 61,032                  \\
	& mkdir-5.2.1                                      &
	34,801                                                    &
	\cellcolor[HTML]{B7B7B7}8,625                     &
	\cellcolor[HTML]{EFEFEF}8,782                      & 8,418                    &
	\cellcolor[HTML]{B7B7B7}3,227                     &
	\cellcolor[HTML]{EFEFEF}2,428                      & 1,877                    &
	\cellcolor[HTML]{B7B7B7}11,969                    &
	\cellcolor[HTML]{EFEFEF}2,836                      & 2,099                   \\
	& rm-8.4                                           &
	44,459                                                    &
	\cellcolor[HTML]{B7B7B7}8,507                     &
	\cellcolor[HTML]{EFEFEF}8,467                      & 8,461                    &
	\cellcolor[HTML]{B7B7B7}12,087                    &
	\cellcolor[HTML]{EFEFEF}5,008                      & 5,109                    &
	\cellcolor[HTML]{B7B7B7}33,171                    &
	\cellcolor[HTML]{EFEFEF}5,097                      & 5,057                   \\
	& sort-8.16                                        &
	88,068                                                    &
	\cellcolor[HTML]{B7B7B7}14,893                    &
	\cellcolor[HTML]{EFEFEF}14,843                     & 15,834                   &
	\cellcolor[HTML]{B7B7B7}60,631                    &
	\cellcolor[HTML]{EFEFEF}61,739                     & 21,948                   &
	\cellcolor[HTML]{B7B7B7}119,150                   &
	\cellcolor[HTML]{EFEFEF}18,711                     & 7,914                   \\
	& tar-1.14                                         &
	163,296                                                   &
	\cellcolor[HTML]{B7B7B7}20,411                    &
	\cellcolor[HTML]{EFEFEF}20,713                     & 20,592                   &
	\cellcolor[HTML]{B7B7B7}115,234                   &
	\cellcolor[HTML]{EFEFEF}95,765                     & 77,910                   &
	\cellcolor[HTML]{B7B7B7}200,394                   &
	\cellcolor[HTML]{EFEFEF}14,384                     & 12,095                  \\
	& uniq-8.16                                        &
	63,861                                                    &
	\cellcolor[HTML]{B7B7B7}14,350                    &
	\cellcolor[HTML]{EFEFEF}14,262                     & 14,354                   &
	\cellcolor[HTML]{B7B7B7}21,672                    &
	\cellcolor[HTML]{EFEFEF}23,177                     & 19,124                   &
	\cellcolor[HTML]{B7B7B7}25,886                    &
	\cellcolor[HTML]{EFEFEF}4,228                      & 3,669                   \\
	\cmidrule(l){2-12}
	\multirow{-11}{*}{\debloatBenchmarkNameShort} &
	\multicolumn{1}{c|}{Mean}                        &
	65,151                                                    &
	\cellcolor[HTML]{B7B7B7}15,080                    &
	\cellcolor[HTML]{EFEFEF}15,152                     & 15,235                   &
	\cellcolor[HTML]{B7B7B7}43,827                    &
	\cellcolor[HTML]{EFEFEF}28,505                     & 21,782                   &
	\cellcolor[HTML]{B7B7B7}72,140                    &
	\cellcolor[HTML]{EFEFEF}11,803                     & 10,686                  \\
	\midrule
	& xml-071d221-1                                    &
	20,090                                                    &
	\cellcolor[HTML]{B7B7B7}10                        &
	\cellcolor[HTML]{EFEFEF}15                         & 20                       &
	\cellcolor[HTML]{B7B7B7}73                        &
	\cellcolor[HTML]{EFEFEF}114                        & 144                      &
	\cellcolor[HTML]{B7B7B7}29                        &
	\cellcolor[HTML]{EFEFEF}50                         & 69                      \\
	& xml-071d221-2                                    &
	20,387                                                    &
	\cellcolor[HTML]{B7B7B7}13                        &
	\cellcolor[HTML]{EFEFEF}14                         & 20                       &
	\cellcolor[HTML]{B7B7B7}155                       &
	\cellcolor[HTML]{EFEFEF}146                        & 243                      &
	\cellcolor[HTML]{B7B7B7}60                        &
	\cellcolor[HTML]{EFEFEF}69                         & 117                     \\
	& xml-1e9bc83-1                                    &
	20,327                                                    &
	\cellcolor[HTML]{B7B7B7}38                        &
	\cellcolor[HTML]{EFEFEF}49                         & 24                       &
	\cellcolor[HTML]{B7B7B7}491                       &
	\cellcolor[HTML]{EFEFEF}522                        & 284                      &
	\cellcolor[HTML]{B7B7B7}235                       &
	\cellcolor[HTML]{EFEFEF}236                        & 115                     \\
	& xml-1e9bc83-2                                    &
	20,222                                                    &
	\cellcolor[HTML]{B7B7B7}79                        &
	\cellcolor[HTML]{EFEFEF}78                         & 76                       &
	\cellcolor[HTML]{B7B7B7}1,391                     &
	\cellcolor[HTML]{EFEFEF}814                        & 867                      &
	\cellcolor[HTML]{B7B7B7}725                       &
	\cellcolor[HTML]{EFEFEF}390                        & 384                     \\
	& xml-1e9bc83-3                                    &
	20,219                                                    &
	\cellcolor[HTML]{B7B7B7}69                        &
	\cellcolor[HTML]{EFEFEF}70                         & 72                       &
	\cellcolor[HTML]{B7B7B7}1,313                     &
	\cellcolor[HTML]{EFEFEF}893                        & 889                      &
	\cellcolor[HTML]{B7B7B7}619                       &
	\cellcolor[HTML]{EFEFEF}416                        & 404                     \\
	& xml-1e9bc83-4                                    &
	19,985                                                    &
	\cellcolor[HTML]{B7B7B7}156                       &
	\cellcolor[HTML]{EFEFEF}139                        & 143                      &
	\cellcolor[HTML]{B7B7B7}3,911                     &
	\cellcolor[HTML]{EFEFEF}1,939                      & 2,521                    &
	\cellcolor[HTML]{B7B7B7}1,943                     &
	\cellcolor[HTML]{EFEFEF}935                        & 1,173                   \\
	& xml-1e9bc83-5                                    &
	20,579                                                    &
	\cellcolor[HTML]{B7B7B7}81                        &
	\cellcolor[HTML]{EFEFEF}73                         & 75                       &
	\cellcolor[HTML]{B7B7B7}1,355                     &
	\cellcolor[HTML]{EFEFEF}929                        & 882                      &
	\cellcolor[HTML]{B7B7B7}746                       &
	\cellcolor[HTML]{EFEFEF}485                        & 428                     \\
	& xml-1e9bc83-6                                    &
	19,880                                                    &
	\cellcolor[HTML]{B7B7B7}127                       &
	\cellcolor[HTML]{EFEFEF}126                        & 124                      &
	\cellcolor[HTML]{B7B7B7}3,563                     &
	\cellcolor[HTML]{EFEFEF}1,852                      & 1,548                    &
	\cellcolor[HTML]{B7B7B7}1,907                     &
	\cellcolor[HTML]{EFEFEF}964                        & 749                     \\
	& xml-1e9bc83-7                                    &
	20,297                                                    &
	\cellcolor[HTML]{B7B7B7}111                       &
	\cellcolor[HTML]{EFEFEF}114                        & 111                      &
	\cellcolor[HTML]{B7B7B7}3,419                     &
	\cellcolor[HTML]{EFEFEF}1,684                      & 2,330                    &
	\cellcolor[HTML]{B7B7B7}1,757                     &
	\cellcolor[HTML]{EFEFEF}827                        & 931                     \\
	& xml-1e9bc83-8                                    &
	20,327                                                    &
	\cellcolor[HTML]{B7B7B7}100                       &
	\cellcolor[HTML]{EFEFEF}107                        & 100                      &
	\cellcolor[HTML]{B7B7B7}2,862                     &
	\cellcolor[HTML]{EFEFEF}1,636                      & 1,446                    &
	\cellcolor[HTML]{B7B7B7}1,451                     &
	\cellcolor[HTML]{EFEFEF}751                        & 592                     \\
	& xml-1e9bc83-9                                    &
	20,330                                                    &
	\cellcolor[HTML]{B7B7B7}128                       &
	\cellcolor[HTML]{EFEFEF}73                         & 128                      &
	\cellcolor[HTML]{B7B7B7}2,850                     &
	\cellcolor[HTML]{EFEFEF}1,230                      & 2,494                    &
	\cellcolor[HTML]{B7B7B7}1,437                     &
	\cellcolor[HTML]{EFEFEF}561                        & 832                     \\
	& xml-2d4ec80-1                                    &
	20,129                                                    &
	\cellcolor[HTML]{B7B7B7}76                        &
	\cellcolor[HTML]{EFEFEF}72                         & 76                       &
	\cellcolor[HTML]{B7B7B7}570                       &
	\cellcolor[HTML]{EFEFEF}522                        & 791                      &
	\cellcolor[HTML]{B7B7B7}384                       &
	\cellcolor[HTML]{EFEFEF}304                        & 354                     \\
	& xml-327c8af-1                                    &
	20,207                                                    &
	\cellcolor[HTML]{B7B7B7}55                        &
	\cellcolor[HTML]{EFEFEF}55                         & 55                       &
	\cellcolor[HTML]{B7B7B7}864                       &
	\cellcolor[HTML]{EFEFEF}625                        & 958                      &
	\cellcolor[HTML]{B7B7B7}527                       &
	\cellcolor[HTML]{EFEFEF}319                        & 392                     \\
	& xml-3398ac2-1                                    &
	20,414                                                    &
	\cellcolor[HTML]{B7B7B7}45                        &
	\cellcolor[HTML]{EFEFEF}44                         & 48                       &
	\cellcolor[HTML]{B7B7B7}345                       &
	\cellcolor[HTML]{EFEFEF}383                        & 605                      &
	\cellcolor[HTML]{B7B7B7}225                       &
	\cellcolor[HTML]{EFEFEF}192                        & 268                     \\
	& xml-3398ac2-2                                    &
	19,290                                                    &
	\cellcolor[HTML]{B7B7B7}48                        &
	\cellcolor[HTML]{EFEFEF}48                         & 48                       &
	\cellcolor[HTML]{B7B7B7}613                       &
	\cellcolor[HTML]{EFEFEF}492                        & 578                      &
	\cellcolor[HTML]{B7B7B7}358                       &
	\cellcolor[HTML]{EFEFEF}255                        & 238                     \\
	& xml-3398ac2-3                                    &
	20,222                                                    &
	\cellcolor[HTML]{B7B7B7}62                        &
	\cellcolor[HTML]{EFEFEF}62                         & 62                       &
	\cellcolor[HTML]{B7B7B7}632                       &
	\cellcolor[HTML]{EFEFEF}574                        & 764                      &
	\cellcolor[HTML]{B7B7B7}347                       &
	\cellcolor[HTML]{EFEFEF}276                        & 306                     \\
	& xml-3398ac2-4                                    &
	19,913                                                    &
	\cellcolor[HTML]{B7B7B7}111                       &
	\cellcolor[HTML]{EFEFEF}112                        & 111                      &
	\cellcolor[HTML]{B7B7B7}1,419                     &
	\cellcolor[HTML]{EFEFEF}1,197                      & 1,722                    &
	\cellcolor[HTML]{B7B7B7}802                       &
	\cellcolor[HTML]{EFEFEF}584                        & 680                     \\
	& xml-3398ac2-5                                    &
	20,477                                                    &
	\cellcolor[HTML]{B7B7B7}44                        &
	\cellcolor[HTML]{EFEFEF}38                         & 44                       &
	\cellcolor[HTML]{B7B7B7}850                       &
	\cellcolor[HTML]{EFEFEF}531                        & 633                      &
	\cellcolor[HTML]{B7B7B7}507                       &
	\cellcolor[HTML]{EFEFEF}269                        & 261                     \\
	& xml-4c99b96-1                                    &
	20,513                                                    &
	\cellcolor[HTML]{B7B7B7}80                        &
	\cellcolor[HTML]{EFEFEF}78                         & 80                       &
	\cellcolor[HTML]{B7B7B7}1,427                     &
	\cellcolor[HTML]{EFEFEF}1,126                      & 1,385                    &
	\cellcolor[HTML]{B7B7B7}699                       &
	\cellcolor[HTML]{EFEFEF}452                        & 438                     \\
	& xml-4c99b96-10                                   &
	20,522                                                    &
	\cellcolor[HTML]{B7B7B7}46                        &
	\cellcolor[HTML]{EFEFEF}47                         & 46                       &
	\cellcolor[HTML]{B7B7B7}1,012                     &
	\cellcolor[HTML]{EFEFEF}760                        & 873                      &
	\cellcolor[HTML]{B7B7B7}443                       &
	\cellcolor[HTML]{EFEFEF}299                        & 256                     \\
	& xml-4c99b96-11                                   &
	19,901                                                    &
	\cellcolor[HTML]{B7B7B7}53                        &
	\cellcolor[HTML]{EFEFEF}54                         & 53                       &
	\cellcolor[HTML]{B7B7B7}868                       &
	\cellcolor[HTML]{EFEFEF}661                        & 791                      &
	\cellcolor[HTML]{B7B7B7}357                       &
	\cellcolor[HTML]{EFEFEF}252                        & 236                     \\
	& xml-4c99b96-12                                   &
	19,775                                                    &
	\cellcolor[HTML]{B7B7B7}102                       &
	\cellcolor[HTML]{EFEFEF}104                        & 102                      &
	\cellcolor[HTML]{B7B7B7}2,429                     &
	\cellcolor[HTML]{EFEFEF}1,592                      & 2,422                    &
	\cellcolor[HTML]{B7B7B7}1,077                     &
	\cellcolor[HTML]{EFEFEF}626                        & 773                     \\
	& xml-4c99b96-13                                   &
	20,114                                                    &
	\cellcolor[HTML]{B7B7B7}60                        &
	\cellcolor[HTML]{EFEFEF}61                         & 60                       &
	\cellcolor[HTML]{B7B7B7}1,132                     &
	\cellcolor[HTML]{EFEFEF}870                        & 989                      &
	\cellcolor[HTML]{B7B7B7}494                       &
	\cellcolor[HTML]{EFEFEF}335                        & 309                     \\
	& xml-4c99b96-14                                   &
	19,970                                                    &
	\cellcolor[HTML]{B7B7B7}102                       &
	\cellcolor[HTML]{EFEFEF}103                        & 102                      &
	\cellcolor[HTML]{B7B7B7}2,147                     &
	\cellcolor[HTML]{EFEFEF}1,687                      & 1,534                    &
	\cellcolor[HTML]{B7B7B7}987                       &
	\cellcolor[HTML]{EFEFEF}600                        & 504                     \\
	& xml-4c99b96-15                                   &
	20,138                                                    &
	\cellcolor[HTML]{B7B7B7}46                        &
	\cellcolor[HTML]{EFEFEF}46                         & 46                       &
	\cellcolor[HTML]{B7B7B7}843                       &
	\cellcolor[HTML]{EFEFEF}788                        & 729                      &
	\cellcolor[HTML]{B7B7B7}381                       &
	\cellcolor[HTML]{EFEFEF}297                        & 244                     \\
	& xml-4c99b96-16                                   &
	20,126                                                    &
	\cellcolor[HTML]{B7B7B7}67                        &
	\cellcolor[HTML]{EFEFEF}68                         & 70                       &
	\cellcolor[HTML]{B7B7B7}1,366                     &
	\cellcolor[HTML]{EFEFEF}1,189                      & 1,125                    &
	\cellcolor[HTML]{B7B7B7}658                       &
	\cellcolor[HTML]{EFEFEF}414                        & 409                     \\
	& xml-4c99b96-17                                   &
	20,210                                                    &
	\cellcolor[HTML]{B7B7B7}67                        &
	\cellcolor[HTML]{EFEFEF}68                         & 70                       &
	\cellcolor[HTML]{B7B7B7}1,360                     &
	\cellcolor[HTML]{EFEFEF}1,310                      & 1,120                    &
	\cellcolor[HTML]{B7B7B7}658                       &
	\cellcolor[HTML]{EFEFEF}414                        & 409                     \\
	& xml-4c99b96-18                                   &
	20,390                                                    &
	\cellcolor[HTML]{B7B7B7}28                        &
	\cellcolor[HTML]{EFEFEF}28                         & 25                       &
	\cellcolor[HTML]{B7B7B7}724                       &
	\cellcolor[HTML]{EFEFEF}492                        & 410                      &
	\cellcolor[HTML]{B7B7B7}324                       &
	\cellcolor[HTML]{EFEFEF}164                        & 137                     \\
	& xml-4c99b96-19                                   &
	20,192                                                    &
	\cellcolor[HTML]{B7B7B7}81                        &
	\cellcolor[HTML]{EFEFEF}82                         & 81                       &
	\cellcolor[HTML]{B7B7B7}1,729                     &
	\cellcolor[HTML]{EFEFEF}1,798                      & 1,895                    &
	\cellcolor[HTML]{B7B7B7}793                       &
	\cellcolor[HTML]{EFEFEF}540                        & 710                     \\
	& xml-4c99b96-2                                    &
	20,750                                                    &
	\cellcolor[HTML]{B7B7B7}53                        &
	\cellcolor[HTML]{EFEFEF}54                         & 53                       &
	\cellcolor[HTML]{B7B7B7}878                       &
	\cellcolor[HTML]{EFEFEF}1,017                      & 912                      &
	\cellcolor[HTML]{B7B7B7}362                       &
	\cellcolor[HTML]{EFEFEF}281                        & 318                     \\
	& xml-4c99b96-3                                    &
	20,015                                                    &
	\cellcolor[HTML]{B7B7B7}67                        &
	\cellcolor[HTML]{EFEFEF}68                         & 67                       &
	\cellcolor[HTML]{B7B7B7}1,102                     &
	\cellcolor[HTML]{EFEFEF}1,254                      & 900                      &
	\cellcolor[HTML]{B7B7B7}483                       &
	\cellcolor[HTML]{EFEFEF}357                        & 337                     \\
	& xml-4c99b96-4                                    &
	20,201                                                    &
	\cellcolor[HTML]{B7B7B7}67                        &
	\cellcolor[HTML]{EFEFEF}67                         & 67                       &
	\cellcolor[HTML]{B7B7B7}1,097                     &
	\cellcolor[HTML]{EFEFEF}1,238                      & 860                      &
	\cellcolor[HTML]{B7B7B7}482                       &
	\cellcolor[HTML]{EFEFEF}365                        & 328                     \\
	& xml-4c99b96-5                                    &
	20,279                                                    &
	\cellcolor[HTML]{B7B7B7}63                        &
	\cellcolor[HTML]{EFEFEF}62                         & 60                       &
	\cellcolor[HTML]{B7B7B7}1,170                     &
	\cellcolor[HTML]{EFEFEF}1,155                      & 1,029                    &
	\cellcolor[HTML]{B7B7B7}515                       &
	\cellcolor[HTML]{EFEFEF}347                        & 364                     \\
	& xml-4c99b96-6                                    &
	19,973                                                    &
	\cellcolor[HTML]{B7B7B7}81                        &
	\cellcolor[HTML]{EFEFEF}82                         & 87                       &
	\cellcolor[HTML]{B7B7B7}1,258                     &
	\cellcolor[HTML]{EFEFEF}1,338                      & 1,056                    &
	\cellcolor[HTML]{B7B7B7}511                       &
	\cellcolor[HTML]{EFEFEF}381                        & 441                     \\
	& xml-4c99b96-7                                    &
	19,973                                                    &
	\cellcolor[HTML]{B7B7B7}115                       &
	\cellcolor[HTML]{EFEFEF}115                        & 115                      &
	\cellcolor[HTML]{B7B7B7}3,399                     &
	\cellcolor[HTML]{EFEFEF}2,560                      & 1,535                    &
	\cellcolor[HTML]{B7B7B7}1,485                     &
	\cellcolor[HTML]{EFEFEF}811                        & 676                     \\
	& xml-4c99b96-8                                    &
	20,579                                                    &
	\cellcolor[HTML]{B7B7B7}42                        &
	\cellcolor[HTML]{EFEFEF}41                         & 42                       &
	\cellcolor[HTML]{B7B7B7}926                       &
	\cellcolor[HTML]{EFEFEF}810                        & 687                      &
	\cellcolor[HTML]{B7B7B7}422                       &
	\cellcolor[HTML]{EFEFEF}254                        & 323                     \\
	& xml-4c99b96-9                                    &
	20,075                                                    &
	\cellcolor[HTML]{B7B7B7}53                        &
	\cellcolor[HTML]{EFEFEF}53                         & 53                       &
	\cellcolor[HTML]{B7B7B7}884                       &
	\cellcolor[HTML]{EFEFEF}940                        & 650                      &
	\cellcolor[HTML]{B7B7B7}368                       &
	\cellcolor[HTML]{EFEFEF}278                        & 265                     \\
	& xml-8ede045-1                                    &
	20,192                                                    &
	\cellcolor[HTML]{B7B7B7}48                        &
	\cellcolor[HTML]{EFEFEF}61                         & 69                       &
	\cellcolor[HTML]{B7B7B7}1,152                     &
	\cellcolor[HTML]{EFEFEF}1,232                      & 1,137                    &
	\cellcolor[HTML]{B7B7B7}499                       &
	\cellcolor[HTML]{EFEFEF}389                        & 487                     \\
	& xml-8ede045-2                                    &
	20,177                                                    &
	\cellcolor[HTML]{B7B7B7}17                        &
	\cellcolor[HTML]{EFEFEF}22                         & 34                       &
	\cellcolor[HTML]{B7B7B7}316                       &
	\cellcolor[HTML]{EFEFEF}335                        & 360                      &
	\cellcolor[HTML]{B7B7B7}132                       &
	\cellcolor[HTML]{EFEFEF}107                        & 164                     \\
	& xml-8ede045-3                                    &
	20,393                                                    &
	\cellcolor[HTML]{B7B7B7}31                        &
	\cellcolor[HTML]{EFEFEF}31                         & 31                       &
	\cellcolor[HTML]{B7B7B7}476                       &
	\cellcolor[HTML]{EFEFEF}431                        & 313                      &
	\cellcolor[HTML]{B7B7B7}199                       &
	\cellcolor[HTML]{EFEFEF}134                        & 134                     \\
	& xml-8ede045-4                                    &
	20,123                                                    &
	\cellcolor[HTML]{B7B7B7}31                        &
	\cellcolor[HTML]{EFEFEF}25                         & 31                       &
	\cellcolor[HTML]{B7B7B7}578                       &
	\cellcolor[HTML]{EFEFEF}472                        & 435                      &
	\cellcolor[HTML]{B7B7B7}250                       &
	\cellcolor[HTML]{EFEFEF}151                        & 181                     \\
	& xml-8ede045-5                                    &
	20,051                                                    &
	\cellcolor[HTML]{B7B7B7}17                        &
	\cellcolor[HTML]{EFEFEF}20                         & 17                       &
	\cellcolor[HTML]{B7B7B7}185                       &
	\cellcolor[HTML]{EFEFEF}246                        & 204                      &
	\cellcolor[HTML]{B7B7B7}61                        &
	\cellcolor[HTML]{EFEFEF}72                         & 80                      \\
	& xml-8ede045-6                                    &
	20,636                                                    &
	\cellcolor[HTML]{B7B7B7}73                        &
	\cellcolor[HTML]{EFEFEF}80                         & 76                       &
	\cellcolor[HTML]{B7B7B7}1,365                     &
	\cellcolor[HTML]{EFEFEF}1,479                      & 1,545                    &
	\cellcolor[HTML]{B7B7B7}552                       &
	\cellcolor[HTML]{EFEFEF}469                        & 700                     \\
	& xml-8ede045-7                                    &
	20,054                                                    &
	\cellcolor[HTML]{B7B7B7}106                       &
	\cellcolor[HTML]{EFEFEF}106                        & 106                      &
	\cellcolor[HTML]{B7B7B7}2,851                     &
	\cellcolor[HTML]{EFEFEF}1,686                      & 1,237                    &
	\cellcolor[HTML]{B7B7B7}1,447                     &
	\cellcolor[HTML]{EFEFEF}614                        & 634                     \\
	& xml-8ede045-8                                    &
	20,177                                                    &
	\cellcolor[HTML]{B7B7B7}76                        &
	\cellcolor[HTML]{EFEFEF}78                         & 76                       &
	\cellcolor[HTML]{B7B7B7}1,397                     &
	\cellcolor[HTML]{EFEFEF}1,327                      & 1,060                    &
	\cellcolor[HTML]{B7B7B7}597                       &
	\cellcolor[HTML]{EFEFEF}449                        & 475                     \\
	& xml-f053486-1                                    &
	20,030                                                    &
	\cellcolor[HTML]{B7B7B7}10                        &
	\cellcolor[HTML]{EFEFEF}10                         & 10                       &
	\cellcolor[HTML]{B7B7B7}101                       &
	\cellcolor[HTML]{EFEFEF}134                        & 76                       &
	\cellcolor[HTML]{B7B7B7}31                        &
	\cellcolor[HTML]{EFEFEF}41                         & 28                      \\
	\cmidrule(l){2-12}
	\multirow{-47}{*}{\xmlBenchmarkNameShort}     &
	\multicolumn{1}{c|}{Mean}                        &
	20,190                                                    &
	\cellcolor[HTML]{B7B7B7}56                        &
	\cellcolor[HTML]{EFEFEF}56                         & 58                       &
	\cellcolor[HTML]{B7B7B7}972                       &
	\cellcolor[HTML]{EFEFEF}819                        & 821                      &
	\cellcolor[HTML]{B7B7B7}453                       &
	\cellcolor[HTML]{EFEFEF}314                        & 327                     \\ \midrule
	All                                           & \multicolumn{1}{c|}{Mean}                        &
	31,989                                                    &
	\cellcolor[HTML]{B7B7B7}233                       &
	\cellcolor[HTML]{EFEFEF}235                        & 237                      &
	\cellcolor[HTML]{B7B7B7}2,999                     &
	\cellcolor[HTML]{EFEFEF}2,189                      & 2,102                    &
	\cellcolor[HTML]{B7B7B7}2,752                     &
	\cellcolor[HTML]{EFEFEF}1,309                      & 1,320                   \\
	\bottomrule
\end{tabular}
}
\end{table*}

==> table/rq1_p_value.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
		\centering
	\caption{
		Comparison between each pairs of algorithms among \ddmin, \probdd
		and \proj.
		Significance tests are performed with the significant improvement
		highlighted in \textbf{bold}.
		\cn{The metric \texttt{change} is not defined?}
	}
	\label{table:rq1_p_value}
	\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}c|cc|cc|cc@{}}
	\toprule
	\multicolumn{1}{l|}{} & \multicolumn{2}{c|}{\probdd vs \ddmin} &
	\multicolumn{2}{c|}{\proj vs \ddmin} & \multicolumn{2}{c}{\proj vs
	\probdd} \\ \cmidrule(l){2-7}
	\multicolumn{1}{l|}{} & change                 & p-value       & change
	& p-value      & change           & p-value           \\ \midrule
	Final size            & 2.40\%                  & 0.71          & 0.06\%                 &
	0.27         & -2.28\%           & 0.38              \\
	Execution time        & \textbf{-25.35\%}       & 5.38E-05      &
	\textbf{-23.84\%}      & 8.43E-05     & 2.02\%            & 0.36              \\
	Query number          & \textbf{-43.65\%}       & 2.82E-03      &
	\textbf{-46.97\%}      & 3.17E-03     & -5.91\%           & 0.06              \\
	\bottomrule
\end{tabular}
}
\end{table}

==> table/rq2_classification.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
		\centering
	\caption{Classification of \ddmin's queries on the results from
	\cBenchmarkNameShort and \xmlBenchmarkNameShort.
    \victor{distribution?}
	}
	\label{table:rq2_classification}
	\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}c|ccc|ccc|ccc@{}}
	\toprule
	\multirow{2}{*}{} & \multicolumn{3}{c|}{Complement} &
	\multicolumn{3}{c|}{Repeated} & \multicolumn{3}{c}{Other} \\
	& Total     & Success   & Ratio   & Total    & Success   & Ratio  & Total  &
	Success & Ratio  \\ \midrule
	C                 & 70,912    & 2         & 0.00\%   & 21,839   & 49        & 0.22\%
	& 38266  & 2525    & 6.60\%  \\
	XML               & 13,928    & 830       & 5.96\%   & 2,991    & 2         &
	0.07\%  & 8,767  & 1485    & 16.94\% \\ \bottomrule
\end{tabular}
}
\end{table}

==> table/rq2_test.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
		\centering
	\caption{Comparison among \ddmin, \probdd, and \proj \wrt
	the number and ratio of queries that either succeed or fail on both
	\cBenchmarkNameShort and \xmlBenchmarkNameShort.
	}
	\label{table:rq2_test}
	\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}ccc|cc|cc@{}}
	\toprule
	\multirow{2}{*}{}    & \multirow{2}{*}{} & \multirow{2}{*}{Total query} &
	\multicolumn{2}{c|}{Successful query} & \multicolumn{2}{c}{Failed query}
	\\
	&                   &                              & number           & ratio           &
	number         & ratio         \\ \midrule
	\multirow{3}{*}{C}   & \ddmin            & 131,031                      & 2,576
	& 1.97\%           & 128,455        & 98.03\%        \\
	& \probdd           & 47,808                       & 2,525            & 5.28\%           &
	45,283         & 94.72\%        \\
	& \proj             & 41,929                       & 2,641            & 6.30\%           &
	39,288         & 93.70\%        \\ \midrule
	\multirow{3}{*}{XML} & \ddmin            & 25,686                       &
	2,317            & 9.02\%           & 23,369         & 90.98\%        \\
	& \probdd           & 13,109                       & 2,315            & 17.66\%          &
	10,794         & 82.34\%        \\
	& \proj             & 12,864                       & 2,384            & 18.53\%          &
	10,480         & 81.47\%        \\ \bottomrule
\end{tabular}
}
\end{table}

==> table/rq3_random.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
		\centering
		\footnotesize
	\caption{Comparison between \probdd and \probddr on
	\cBenchmarkNameShort and \xmlBenchmarkNameShort.
	}
	\label{table:rq3_random}
    \renewcommand{\arraystretch}{.8}
%	\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}c|ccc|ccc@{}}
	\toprule
	\multicolumn{1}{l|}{} & \multicolumn{3}{c|}{C}  & \multicolumn{3}{c}{XML}
	\\
	\multicolumn{1}{l|}{} & Size  & Time   & Query  & Size  & Time   & Query
	\\
	\midrule
	\probdd               & 575.9 & 2,582.2 & 7,436.6 & 56.7  & 671.3  & 292.7  \\
	\probddr              & 571.9 & 2,547.1 & 7,747.7 & 56.9  & 676.9  & 301.3  \\
	\midrule
	p-value               & 0.75  & 0.66   & 0.34   & 0.27  & 0.31   & 0.26   \\
	\bottomrule
\end{tabular}
%}
\end{table}

==> table/running_example_results.tex <==
\begin{figure}[ht]
	\centering
	\begin{subtable}{0.48\textwidth}
		\centering
		% First tabular
		\begin{tabular}{r|cccccccc|l}
			test & \myelement{1} & \myelement{2} & \myelement{3} & \myelement{4} & \myelement{5} & \myelement{6} & \myelement{7} & \myelement{8} &   \\ \hline
			1    & \myelement{1} & \myelement{2} & \myelement{3} & \myelement{4} & .  & .  & .  & .  & F \\
			2    & .  & .  & .  & .  & \myelement{5} & \myelement{6} & \myelement{7} & \myelement{8} & F \\ \hline
			3    & \myelement{1} & \myelement{2} & .  & .  & .  & .  & .  & .  & F \\
			4    & .  & .  & \myelement{3} & \myelement{4} & .  & .  & .  & .  & F \\
			5    & .  & .  & .  & .  & \myelement{5} & \myelement{6} & .  & .  & F \\
			6    & .  & .  & .  & .  & .  & .  & \myelement{7} & \myelement{8} & F \\ \hline
			7    & .  & .  & \myelement{3} & \myelement{4} & \myelement{5} & \myelement{6} & \myelement{7} & \myelement{8} & F \\
			8    & \myelement{1} & \myelement{2} & .  & .  & \myelement{5} & \myelement{6} & \myelement{7} & \myelement{8} & F \\
			9    & \myelement{1} & \myelement{2} & \myelement{3} & \myelement{4} & .  & .  & \myelement{7} & \myelement{8} & F \\
			10   & \myelement{1} & \myelement{2} & \myelement{3} & \myelement{4} & \myelement{5} & \myelement{6} & .  & .  & F \\ \hline
			11   & \myelement{1} & .  & .  & .  & .  & .  & .  & .  & F \\
			12   & .  & \myelement{2} & .  & .  & .  & .  & .  & .  & F \\
			13   & .  & .  & \myelement{3} & .  & .  & .  & .  & .  & F \\
			14   & .  & .  & .  & \myelement{4} & .  & .  & .  & .  & F
		\end{tabular}
		\caption{\ddmin, first half}
		\label{table:running_example_results_ddmin_first_half}
	\end{subtable}%
	\hfill
	\begin{subtable}{0.48\textwidth}
		\centering
		% Second tabular
		\begin{tabular}{r|cccccccc|l}
			15 & .  & .  & .  & .  & \myelement{5}                       & .  & .  & .  & F \\
			16 & .  & .  & .  & .  & .                        & \myelement{6} & .  & .  & F \\
			17 & .  & .  & .  & .  & .                        & .  & \myelement{7} & .  & F \\
			18 & .  & .  & .  & .  & .                        & .  & .  & \myelement{8} & F \\ \hline
			19 & .  & \myelement{2} & \myelement{3} & \myelement{4} & \myelement{5}                       & \myelement{6} & \myelement{7} & \myelement{8} & F \\
			20 & \myelement{1} & .  & \myelement{3} & \myelement{4} & \myelement{5}                       & \myelement{6} & \myelement{7} & \myelement{8} & F \\
			21 & \myelement{1} & \myelement{2} & .  & \myelement{4} & \myelement{5}                       & \myelement{6} & \myelement{7} & \myelement{8} & F \\
			22 & \myelement{1} & \myelement{2} & \myelement{3} & .  & \myelement{5}                       & \myelement{6} & \myelement{7} & \myelement{8} & F \\
			23 & \myelement{1} & \myelement{2} & \myelement{3} & \myelement{4} & .                        & \myelement{6} & \myelement{7} & \myelement{8} & T \\ \hline
			24 & .  & \myelement{2} & \myelement{3} & \myelement{4} & \cellcolor[HTML]{C0C0C0} & \myelement{6} & \myelement{7} & \myelement{8} & F \\
			25 & \myelement{1} & .  & \myelement{3} & \myelement{4} & \cellcolor[HTML]{C0C0C0} & \myelement{6} & \myelement{7} & \myelement{8} & F \\
			26 & \myelement{1} & \myelement{2} & .  & \myelement{4} & \cellcolor[HTML]{C0C0C0} & \myelement{6} & \myelement{7} & \myelement{8} & F \\
			27 & \myelement{1} & \myelement{2} & \myelement{3} & .  & \cellcolor[HTML]{C0C0C0} & \myelement{6} & \myelement{7} & \myelement{8} & F \\
			28 & \myelement{1} & \myelement{2} & \myelement{3} & \myelement{4} & \cellcolor[HTML]{C0C0C0} & .  & \myelement{7} & \myelement{8} & F \\
			29 & \myelement{1} & \myelement{2} & \myelement{3} & \myelement{4} & \cellcolor[HTML]{C0C0C0} & \myelement{6} & .  & \myelement{8} & F \\
			30 & \myelement{1} & \myelement{2} & \myelement{3} & \myelement{4} & \cellcolor[HTML]{C0C0C0} & \myelement{6} & \myelement{7} & .  & F \\ \hline
		\end{tabular}
		\caption{\ddmin, second half}
		\label{table:running_example_results_ddmin_second_half}
	\end{subtable}%
	\vfill
	\begin{subtable}{0.48\textwidth}
		\centering
		% Third tabular
		\setlength{\tabcolsep}{2.2pt}
		\begin{tabular}{r|cccccccc|l}
			test                & \myelement{1}                       & \myelement{2}                       & \myelement{3}                       & \myelement{4}                       & \myelement{5}   & \myelement{6}                       & \myelement{7}                       & \myelement{8}   &                     \\
			p                   & 0.25                     & 0.25                     & 0.25                     & 0.25                     & 0.25 & 0.25                     & 0.25                     & 0.25 &                     \\ \hline
			& .                        & \myelement{2}                       & \myelement{3}                       & .                        & .    & \myelement{6}                       & \myelement{7}                       & .    &                     \\
			\multirow{-2}{*}{1} & 0.37                     & 0.25                     & 0.25                     & 0.37                     & 0.37 & 0.25                     & 0.25                     & 0.37 & \multirow{-2}{*}{F} \\ \hline
			& \myelement{1}                       & .                        & .                        & \myelement{4}                       & \myelement{5}   & .                        & .                        & \myelement{8}   &                     \\
			\multirow{-2}{*}{2} & 0.37                     & 0                        & 0                        & 0.37                     & 0.37 & 0                        & 0                        & 0.37 & \multirow{-2}{*}{T} \\ \hline
			& .                        & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \myelement{4}                       & .    & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \myelement{8}   &                     \\
			\multirow{-2}{*}{3} & 0.61                     & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & 0.37                     & 0.61 & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & 0.37 & \multirow{-2}{*}{F} \\ \hline
			& \myelement{1}                       & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & .                        & \myelement{5}   & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & .    &                     \\
			\multirow{-2}{*}{4} & 0.61                     & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & 0.61                     & 0.61 & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & 0.61 & \multirow{-2}{*}{F} \\ \hline
			& \myelement{1}                       & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & .                        & \myelement{5}   & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \myelement{8}   &                     \\
			\multirow{-2}{*}{5} & 0.61                     & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & 0                        & 0.61 & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & 0.61 & \multirow{-2}{*}{T} \\ \hline
			& \myelement{1}                       & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & .    & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \myelement{8}   &                     \\
			\multirow{-2}{*}{6} & 0.61                     & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & 1    & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & 0.61 & \multirow{-2}{*}{F} \\ \hline
			& .                        & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \myelement{5}   & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \myelement{8}   &                     \\
			\multirow{-2}{*}{7} & 0                        & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & 1    & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & 0.61 & \multirow{-2}{*}{T} \\ \hline
			& \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \myelement{5}   & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & .    &                     \\
			\multirow{-2}{*}{8} & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & 1    & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & 1    & \multirow{-2}{*}{F} \\ \hline
		\end{tabular}
		\caption{\probdd}
		\label{table:running_example_results_probdd}
	\end{subtable}%
	\hfill
	\begin{subtable}{0.48\textwidth}
		\centering
		% Fourth tabular
		\begin{tabular}{r|cccccccc|l}
			test                & \myelement{1}                       & \myelement{2}                       & \myelement{3}                       & \myelement{4}                       & \myelement{5} & \myelement{6}                       & \myelement{7}                       & \myelement{8} &                     \\
			c                   & 0                        & 0                        & 0                        & 0                        & 0  & 0                        & 0                        & 0  &                     \\ \hline
			& .                        & \myelement{2}                       & \myelement{3}                       & .                        & .  & \myelement{6}                       & \myelement{7}                       & .  &                     \\
			\multirow{-2}{*}{1} & 1                        & 0                        & 0                        & 1                        & 1  & 0                        & 0                        & 1  & \multirow{-2}{*}{F} \\ \hline
			& \myelement{1}                       & .                        & .                        & \myelement{4}                       & \myelement{5} & .                        & .                        & \myelement{8} &                     \\
			\multirow{-2}{*}{2} & 1                        & -                        & -                        & 1                        & 1  & -                        & -                        & 1  & \multirow{-2}{*}{T} \\ \hline
			& .                        & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \myelement{4}                       & .  & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \myelement{8} &                     \\
			\multirow{-2}{*}{3} & 2                        & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & 1                        & 2  & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & 1  & \multirow{-2}{*}{F} \\ \hline
			& \myelement{1}                       & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & .                        & \myelement{5} & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & .  &                     \\
			\multirow{-2}{*}{4} & 2                        & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & 2                        & 2  & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & 2  & \multirow{-2}{*}{F} \\ \hline
			& \myelement{1}                       & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & .                        & \myelement{5} & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \myelement{8} &                     \\
			\multirow{-2}{*}{5} & 2                        & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & -                        & 2  & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & 2  & \multirow{-2}{*}{T} \\ \hline
			& \myelement{1}                       & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & .  & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \myelement{8} &                     \\
			\multirow{-2}{*}{6} & 2                        & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & 2  & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & 2  & \multirow{-2}{*}{F} \\ \hline
			& .                        & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \myelement{5} & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \myelement{8} &                     \\
			\multirow{-2}{*}{7} & -                        & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & 2  & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & 2  & \multirow{-2}{*}{T} \\ \hline
			& \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \myelement{5} & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & .  &                     \\
			\multirow{-2}{*}{8} & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & 2  & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & 2  & \multirow{-2}{*}{F} \\ \hline
		\end{tabular}
		\caption{\myalgorithm}
		\label{table:running_example_results_myalgorithm}
	\end{subtable}
	\caption{Step-by-step outcomes on \ddmin, \probdd, \myalgorithm on the running example.
		In these table, each line represents a variant with passing or failing the property.
		The first and last column indicate the current test number and test result separately.
		the symbols ``.'' denotes the removal attempt of an element,
        while empty cell with grey background signifies that the element has been confirmed as removable and subsequently removed.
        \victor{did we introduce ``temporary'' and ``permanent'' removal anywhere?} \mz{"attempts to remove" means we temporarily remove something and test}
        \victor{you need to explain this...}
		``T'' and ``F'' indicate whether or not the list retains the specified property.
        In (d), ``-'' means the counter of current element being unavailable,
        as this element has been deleted.
        \victor{I think we should transpose these tables.}\mz{do I need to make \probdd table and \myalgorithm table side by side}
        \victor{we can put three tables row by row. which is better than this.}
		}
	\label{table:running_example_results}
\end{figure}

